Self-Evolving Multi-Agent Collaboration Networks for Software Development

LLM-driven multi-agent collaboration (MAC) systems have demonstrated impressive capabilities in automatic software development at the function level. However, their heavy reliance on human design limits their adaptability to the diverse demands of real-world software development. To address this limitation, we introduce EvoMAC, a novel self-evolving paradigm for MAC networks. Inspired by traditional neural network training, EvoMAC obtains text-based environmental feedback by verifying the MAC network's output against a target proxy and leverages a novel textual backpropagation to update the network. To extend coding capabilities beyond function-level tasks to more challenging software-level development, we further propose rSDE-Bench, a requirement-oriented software development benchmark, which features complex and diverse software requirements along with automatic evaluation of requirement correctness. Our experiments show that: i) The automatic requirement-aware evaluation in rSDE-Bench closely aligns with human evaluations, validating its reliability as a software-level coding benchmark. ii) EvoMAC outperforms previous SOTA methods on both the software-level rSDE-Bench and the function-level HumanEval benchmarks, reflecting its superior coding capabilities. The benchmark can be downloaded at https://yuzhu-cai.github.io/rSDE-Bench/.

==> EvoMAC/content/00-abstract.tex <==
\begin{abstract}
LLM-driven multi-agent collaboration (MAC) systems have demonstrated impressive capabilities in automatic software development at the function level. However, their heavy reliance on human design limits their adaptability to the diverse demands of real-world software development.
To address this limitation, we introduce EvoMAC, a novel self-evolving paradigm for MAC networks. Inspired by traditional neural network training, EvoMAC obtains text-based environmental feedback by verifying the MAC network's output against a target proxy and leverages a novel textual backpropagation to update the network.
To extend coding capabilities beyond function-level tasks to more challenging software-level development, we further propose rSDE-Bench, a requirement-oriented software development benchmark, which features complex and diverse software requirements along with automatic evaluation of requirement correctness.
Our experiments show that:
i) The automatic requirement-aware evaluation in rSDE-Bench closely aligns with human evaluations, validating its reliability as a software-level coding benchmark.
ii) EvoMAC outperforms previous SOTA methods on both the software-level rSDE-Bench and the function-level HumanEval benchmarks, reflecting its superior coding capabilities. The benchmark can be downloaded at \href{https://yuzhu-cai.github.io/rSDE-Bench/}{https://yuzhu-cai.github.io/rSDE-Bench/}.
\end{abstract}

==> EvoMAC/content/01-introduction.tex <==
\vspace{-4mm}
\section{Introduction}
\vspace{-2mm}

Automatic software development focuses on generating code from natural language requirements. 
Code is a universal problem-solving tool, and this automation presents significant potential to provide substantial benefits across all areas of our lives~\cite{Li2022CompetitionlevelCG}.
Recently, the industry has introduced several large language model (LLM)-driven coding assistants, including Microsoft's Copilot~\cite{Copilot}, Amazon's CodeWhisperer~\cite{CodeWhisperer}, and Google's Codey~\cite{Codey}. These coding assistants significantly advance human efficiency and yield considerable commercial benefits. Despite the initial success of LLMs in assisting with line-level coding, they struggle to tackle more complex coding tasks. This limitation stems from the restricted reasoning abilities of single LLMs and their lack of capacity for long-context understanding~\cite{wang2024adaleval,li2024looglelongcontextlanguagemodels,wang2024limitssurveytechniquesextend}.

To handle function-level coding tasks, numerous multiple language agent collaboration (MAC) systems have been proposed~\cite{li2023camel,metagpt2023,chanchateval,mapcoder2024,Yang2024SWEagentAI,Li_2022,GPTEngineer}. These MAC systems function as LLM-driven agentic workflow.
They follow human-designed standardized operating procedures to divide the complex coding tasks into simpler subtasks within the workflow, allowing each agent to conquer specific subtasks.
These MAC systems significantly advance coding capabilities from line-level to function-level tasks.  However, current MAC systems rely on heuristic designs. 
These human-crafted static systems have two inherent limitations: 
i) their performance is confined to human initialization. Given the diversity of real-world coding tasks, human design cannot fully address the specific needs of each task; and
ii) they lack the flexibility to adapt to new tasks. This rigidity necessitates that researchers and developers manually decompose tasks and create prompts. The complexity of this process inhibits effective human optimization for adapting to new challenges.

To address these limitations, we present EvoMAC, a novel self-evolving paradigm for MAC networks. EvoMAC's key feature is its ability to iteratively adapt both agents and their connections during test time for each task. 
Inspired from the standard neural network training, the core idea of self-evolution is to obtain text-based environmental feedback by verifying the MAC network's generation against a target proxy, then leverage a novel textual back-propagation to update the MAC network. Following this general paradigm, we specify EvoMAC for software development, which comprises three essential components: i) an adaptable MAC network-based coding team that generates code through feed-forward; ii) a specifically designed testing team that creates unit test cases serving as the target proxy and verifies the generated code in the compiler to produce objective feedback; and iii) an updating team that uses the textual back-propagation algorithm to update the coding team. By cycling these three components, the coding team can iteratively evolve and generate codes that are better aligned with the unit test cases, eventually fulfilling more  requirements of the coding task.

Our self-evolving MAC network has the potential to further advance coding capabilities from function-level to more complex software-level tasks. As it can iteratively address lengthier task requirements and cater to realistic software development demands. However, existing benchmarks typically focus on specific individual functions~\cite{humaneval2021,mbpp2021,CodeScore,xcodeeval} or bug-fixing~\cite{swebench2023}, leaving a significant gap in providing comprehensive requirements for software development. This gap makes it difficult to fully assess the potential of our self-evolving MAC network.

To support the development of software-level coding capabilities, we propose rSDE-Bench, a novel requirement-oriented software development benchmark. 
It is the first benchmark that features both complex and diverse software requirements, as well as the automatic evaluation of requirement correctness. rSDE-Bench involves 53 coding tasks with 616 requirements, covering two typical software types, Website, and Game, and two requirement difficulty levels, Basic and Advanced.  Each coding task consists of two components: i) multiple requirements that clearly outline measurable software functionalities, item by item, and ii) paired black-box test cases that automatically verify the correctness of each requirement. 
rSDE-Bench can achieve automatic evaluation with these synchronized pairs of requirements and test cases.
The rSDE-Bench introduces new software-level challenges, including lengthy requirement analysis and long-context coding, which are essential in real-world software development but are absent in existing benchmarks.
% \Note{sc: one sentence for automatic evaluation}

To validate the effectiveness of our proposed EvoMAC and rSDE-Bench, we conduct three key evaluations. 
First, we compare our automatic evaluation in rSDE-Bench with human evaluation, achieving a coherence score of 99.22\%, demonstrating its reliability. 
Second, we compare EvoMAC against five multi-agent and three single-agent baselines. EvoMAC significantly outperforms previous SOTAs by 26.48\%, 34.78\%, and 6.10\% on Website Basic, Game Basic, and HumanEval, respectively, underscoring its effectiveness. Third, we evaluate EvoMAC with varying evolving times and two different driving LLMs. The results indicate that EvoMAC consistently improves with more evolving times and shows convincing enhancements regardless of the driving LLM used, further demonstrating the effectiveness of our self-evolving design.

To sum up, our contributions are:

$\bullet$ We propose EvoMAC, a novel self-evolving MAC network, and apply it to software development. EvoMAC can iteratively adapt both agents and their connections during test time for each task. 

$\bullet$ We propose rSDE-Bench, a novel requirement-oriented software development benchmark. It is the first benchmark that features both complex and diverse software requirements, as well as the automatic evaluation of requirement correctness.

$\bullet$ We conduct comprehensive experiments and validate that: automatic evaluation in rSDE-Bench is highly aligned with human evaluation; EvoMAC outperforms previous SOTAs, and self-evolving promises continuous improvement with evolving times.


% To enable automatic software development, previous works have made efforts
% from two aspects. From the system perspective, numerous multiple language agent collaboration (MAC) systems~\cite{metagpt2023,chanchateval,mapcoder2024,Yang2024SWEagentAI} have been proposed. They follow human-designed standardized operating procedures to divide the complex coding task into manageable subtasks within LLM agent pipelines, allowing each agent to conquer specific aspects efficiently. 
% From the benchmark perspective, a variety of coding tasks have been established to test and refine these developments. They mainly focus on function completion~\cite{humaneval2021,mbpp2021} and bug repairing~\cite{swebench2023}.
% These MAC systems achieve promising results on existing benchmarks.
% , demonstrating over 90\% success rate in function completion~\cite{humaneval2021} and 45\% in bug fixing task~\cite{swebench2023}

% , which requires completing a function given its description, ii) , which requires fixing a specified bug within the code context.

% , and ii) software development~\cite{metagpt2023,chatdev2023}, which requires developing a software given the human language description.
% , which are constrained by human initialization. Historical trends in machine learning show that manually crafted solutions are often superseded by more efficient learned alternatives. Second, existing benchmarks typically emphasize only a single requirement, such as a specific function or issue description. In the real world, software requirements are much more complicated, encompassing various application types (such as GUIs and websites), interaction methods (like keyboard and mouse), and complex logical rules (such as games and file management). To bridge this gap and approach realistic software development capabilities, we emphasize two critical components: dynamic MAC networks and benchmarks grounded in real-world requirements. 

% Despite this promising progress, there remains a substantial gap between the capabilities of current MAC systems and the demands of real-world software development. In practice, software development often involves complex and lengthy requirements, requiring teams of expert programmers to work continuously for months or even years. 
% Current MAC systems are built on heuristic designs and lack the iterative capabilities essential for tackling the challenges of realistic software development. Existing benchmarks typically focus on single requirements, such as a specific function or bug, which do not adequately provide the comprehensive requirements in software development.
% To bridge this gap and develop the MAC system to approach realistic software development capabilities, we emphasize two critical components: dynamic MAC system and requirement-oriented software development benchmarks. 

% \NoteYhu{More concrete and scientific expression.}


% From the system perspective, we propose EvoMAC, a novel self-evolving MAC network and its application to software development. The key feature of EvoMAC is its ability to iteratively adapt both agents and their connections during test time for each task. 
% The key idea for evolving during test time is to set up a target proxy and introduce objective environment feedback, which verifies the generated output against the target proxy and guides improvements. This process is akin to the network training.
% Following this general recipe, we implement the self-evolving MAC network for software development, comprising three essential elements: i) a learnable MAC network-based coding team that feeds forward and generates code; ii) a specifically designed testing team that creates test cases serving as the target proxy, with the generated code verified in the compiler to produce objective feedback; and iii) an updating team that employs a novel textual back-propagation algorithm to refine the coding team. By cycling these three parts, the coding team can iteratively evolve. Then the generated code can be better aligned with the test cases, this is, fulfilling more task requirements.

% From the benchmark perspective, we propose rSDE-Bench, a novel requirement-oriented software development benchmark. It is the first benchmark that features both complex and diverse software requirements, as well as the automatic evaluation of requirement correctness. Each task sample consists of two components: i) multiple requirements that clearly outline measurable software functionalities, item by item, and ii) paired black-box test cases that automatically verify the correctness of each requirement. To further enrich the diversity, rSDE-Bench involves two typical software types, Website, and Game, two language types, Python and HTML, and two difficulty levels, Basic and Advanced. rSDE-Bench introduces new challenges, including lengthy requirement analysis and long-context coding, which are essential in real-world software development but are absent in existing benchmarks.


% To validate the effectiveness of our proposed EvoMAC and rSDE-Bench, we conduct three key evaluations. 
% First, we compare our automatic evaluation in rSDE-Bench with human evaluation, achieving a coherence score of 0.9922, demonstrating its effectiveness. 
% Second, we compare EvoMAC against five multi-agent and three single-agent baselines. EvoMAC significantly outperforms previous SOTAs by 26.48\%, 34.78\%, and 6.10\% on Website Basic, Game Basic, and HumanEval, respectively, underscoring its effectiveness. 
% Third, we evaluate EvoMAC with varying evolving times and two different models. The results indicate that EvoMAC consistently improves with increased evolving times and shows reliable enhancements regardless of the LLM drives used, further demonstrating the effectiveness of our self-evolving design.

% To sum up, our contributions are:

% $\bullet$ We propose EvoMAC, a novel self-evolving MAC network and its application to software development. EvoMAC can iteratively adapt both agents and their connections during test time for each task. 

% $\bullet$ We propose rSDE-Bench, a novel requirement-oriented software development benchmark. It is the first benchmark that features both complex and diverse software requirements, as well as the automatic evaluation of requirement correctness.

% $\bullet$ we conduct comprehensive experiments and validate that: automatic evaluation in rSDE-Bench is highly aligned with human evaluation; EvoMAC outperforms previous SOTAs, and self-evolving promises continuous improvement with iteration times regardless of the LLM drives used.

% becomes increasingly aligned with the test cases which specifies the conditions of task requirements. Evolving toward this target proxy can lead to improved task completion.

% , ultimately leading to enhanced completion of coding tasks.

% The target proxy defines the conditions for 

% The MAC network is implemented with structured coding agents. The target proxy is achieved with test cases, the objective feedback is achieved by compiler execution results. The key is to iteratively refine the MAC network to fix the issues in the current generation. To achieve this, we propose a novel textual back-propagation algorithm. It has two steps: i) the gradient agent evaluates the task completion levels of each coding agent based on the execution logs, and ii) following this analysis, the updating agent revises the agent prompts and connections accordingly. This textual back-propagation algorithm enables the MAC network to iteratively evolve to be more closely aligned with the test cases, ultimately leading to improved coding task completion.






% These MAC networks achieve promising results, demonstrating over 90\% success rate in code completion tasks~\cite{humaneval2021} and 45\% in realistic GitHub bug fixing tasks~\cite{swebench2023}. \NoteYhu{Thinking: more focused on software development achievements? More description about why use MAC.}









% However, with the rapid advancement of language agents and the compound agentic system, existing benchmarks .  which limits its ability to reflect the current capabilities and limitations of state-of-the-art language models.

% Language agents like GPTs, Claude, LLaMA, and Gemini commonly use the HumanEval code completion benchmark to demonstrate their skills. 
% To improve the 
% Orthogonal to improving individual language agent capability, recent multiple language agent collaboration networks 

% Besides monolithic model query, recent  demonstrated 


% This 'divide-and-conquer' strategy is commonly employed in human collaboration and accumulated as (SOPs). Numerous MAC networks that heuristically replicate these human-designed SOPs using agents are proposed~\cite{MetaGPT,MAPCoder,AgentCoder,ChatDEV}, Numerous MAC networks that heuristically replicate these human-designed SOPs using agents are proposed~\cite{MetaGPT,MAPCoder,AgentCoder,ChatDEV}
% A representative task is software development, which demands diverse skills, such as strong reasoning, planning, and long context processing capability to synthesize code from natural language requirements. 






% [Multi-agent is important] Recent advances in large language models open the possibility of general task process. They can process diverse tasks, ranging from math, qa, and coding. 
% Despite their advancements, solving more complex problems reliably often requires a compound agentic system with multiple components instead of a monolithic model query. 
% They can be achieved as multi-agent collaboration or call a single agent multiple times. 


% [Existing multi-agent collaboration relies on heuristic design.] 


% [We propose automatic self-evolving via textual back-propagation.] 

% The advantages are. 

% To better validate the algorithm, we focus on the software development task. However, the existing software develop benchmarks either rely on human evaluation or . To fill this gap, we propose a benchmark.

% We validate the performance on ***.

==> EvoMAC/content/02-relatedworks.tex <==
\vspace{-4mm}
\section{Related Works}
\vspace{-3mm}
\noindent\textbf{LLM-based multi-agent collaboration.} LLM-driven multi-agent collaboration (MAC) systems~\cite{werewolf2023, waragent2023, ziems2024can, autogen2023, metagpt2023, chanchateval, mandi2024roco} enable multiple agents to share information and collaboratively complete the overall task. These MAC systems function as agentic workflows. They have demonstrated enhanced problem-solving capabilities in various domains, such as mathematics~\cite{mapcoder2024}, software development~\cite{chatdev2023, metagpt2023}, embodied task~\cite{roco2024} and social simulation~\cite{ziems2024can, matrix2024, agenthospital}. However, these systems~\cite{autogen2023, agentverse2023} heavily rely on manually designed workflows, which lack generalizability and the labor-intensive nature of manual design poses significant limitations. To address this issue, we propose a novel self-evolving paradigm, which allows agents to update and improve through external feedback, enabling dynamic adaptation and more advanced performance across varied tasks.
% lack of generalizability and the labor-intensive nature of manual design pose significant limitations. 2) Self-organizing multi-agent systems~\cite{soa2024, kambhampati2024llms} provide agents with the ability to autonomously organize themselves. Despite this, such systems are constrained by the inherent limitations of individual agents and cannot evolve based on feedback, limiting their adaptability. 3) Self-evolving systems allow agents to update and improve either through external feedback or self-summarization. For instance, Symbolic~\cite{symbolic2024} formulates the multi-agent system as a neural network where agent prompts are treated as learnable parameters that can be adjusted. Similarly, DyLAN~\cite{dylan2024} enables dynamic adjustments to the system’s structure by filtering agents within the network. However, these works lack objective feedback and are prone to hallucinations~\cite{hallucination2023}, leading to self-collapse~\cite{theory2023, software_survey2024}. To address these challenges, we propose integrating more objective feedback from the environment and introducing a supervised learning formulation to enable dynamic updates in self-evolving multi-agent systems.

% ############################# 10.1 2:00 ###################################
% \noindent\textbf{LLM-based multi-agent collaboration.} The collaboration of multiple agents based on LLMs enables multi-agent groups to make distributed decisions and execute corresponding actions to achieve common goals, demonstrating enhanced problem-solving capabilities in various tasks.~\cite{werewolf2023, waragent2023, ziems2024can, autogen2023, metagpt2023, chanchateval, mandi2024roco} Current multi-agent work can be divided into three types: manually-designed, self-organizing and self-evolving systems. 1) Manually-designed systems have demonstrated the potential for collaboration in domains such as mathematics~\cite{mapcoder2024}, software development~\cite{chatdev2023, metagpt2023}, and social simulation~\cite{ziems2024can, matrix2024}. These systems assign specific roles to agents and optimize workflows to fully leverage multi-agent capabilities. However, their lack of generalizability and the labor-intensive nature of manual design pose significant limitations. 2) Self-organizing multi-agent systems~\cite{soa2024, kambhampati2024llms} provide agents with the ability to autonomously organize themselves. Despite this, such systems are constrained by the inherent limitations of individual agents and cannot evolve based on feedback, limiting their adaptability. 3) Self-evolving systems allow agents to update and improve either through external feedback or self-summarization. For instance, Symbolic~\cite{symbolic2024} formulates the multi-agent system as a neural network where agent prompts are treated as learnable parameters that can be adjusted. Similarly, DyLAN~\cite{dylan2024} enables dynamic adjustments to the system’s structure by filtering agents within the network. However, these works lack objective feedback and are prone to hallucinations~\cite{hallucination2023}, leading to self-collapse~\cite{theory2023, software_survey2024}. To address these challenges, we propose integrating more objective feedback from the environment and introducing a supervised learning formulation to enable dynamic updates in self-evolving multi-agent systems.



% 问题：要不要在这里引入multi-agent neural network？

% 基于大语言模型的多智能体协作使得多智能体群体能够以分布式的方式共同做出决策并执行相应的行动，以实现共同目标，并在各种任务中展示出增强的问题解决能力。现有的多智能体工作可以分成两种类型：人工设计和动态的多智能体协作，包括自组织和自进化。人工设计的多智能体网络展示了多智能体协作在数学（MapCoder）、软件开发、以及通用问答任务（GAIA）中，通过设定合适的智能体角色以及优化工作流程，可以充分发挥多智能体的能力。但人工设计的多智能体系统缺乏泛化能力且消耗人工。
% 自组织形式的多智能体工作允许多智能体有一定的组织能力，但这些自组织往往受限于本身模型的能力，缺乏根据环境反馈进行优化的能力。自进化的多智能体系统，Symbolic将多智能体系统建模为一个神经网络，并提出该网络的可学习参数是智能体的提示，它可以通过外界反馈或自我总结完成参数更新。DyLAN则是通过筛选多智能体网络中的智能体来实现结构的动态调整。但是这些工作缺乏客观反馈，容易受到幻觉影响，陷入自我崩溃。因此，我们在这篇文章中试图从监督学习的角度定义多智能体系统的更新机制，建立一个自我学习的动态多智能体系统。

% Original version by Dr. Hu
 % LLM-based multi-agent collaboration has garnered significant attention in both industry and academia. These systems enable the multi-agent group collaboratively make decisions and execute corresponding actions in a distributed manner to achieve the common goal and showcase enhanced problem-solving capabilities. They demonstrate superior performance on various tasks, ranging from social simulation to practical problems. For instance, MetaGPT for software generation tasks, MapCoder for code completion, Math-Multi-Agent for math tasks, and FORD for general question-answering tasks (GAIA), CoELA for embodied tasks. However, most existing approaches focus on heuristic and static system designs, with their performance constrained by human-defined initialization. To overcome these limitations, we propose **, a framework that integrates forward and textual backpropagation processes, enabling continuous automatic optimization of multi-agent collaboration networks.


\noindent\textbf{Software development benchmarks.} Software development benchmarks aim to evaluate models in the task of generating code from natural language descriptions~\cite{Zheng2023TowardsAU}. These benchmarks typically include task definitions and evaluation criteria. Existing benchmarks can be categorized into three types: i) function completion (HumanEval~\cite{humaneval2021}, MBPP~\cite{mbpp2021}, EvalPlus~\cite{evalplus}, xCodeEval~\cite{xcodeeval}); ii) bug repair (SWE-bench~\cite{swebench2023}); and iii) software generation (SRDD~\cite{chatdev2023}, SoftwareDev~\cite{metagpt2023}).
Function completion and bug repair benchmarks are confined to function-level task definitions, missing the diverse realistic software requirements. Software generation benchmarks often depend on expensive human evaluations or indirect similarity-based measurements, unable to automatically and accurately verify the requirement correctness.
To address these limitations, we introduce rSDE-Bench, the first benchmark contains both diverse software requirements and automatic evaluation of requirement correctness. It can support the development of more realistic software-level coding capabilities.

% While these benchmarks provide valuable insights into a model’s ability to generate code or fix bugs, they fail to evaluate a model's software development capabilities from the perspective of user requirements. This is fundamental to the entire software development process because requirements define the necessary functions and features of the software, providing clear goals for design and implementation. For instance, SoftwareDev~\cite{metagpt2023} lacks detailed descriptions of the required functions and evaluates semantic metrics like similarity, which fail to accurately measure whether the software meets its intended requirement. To address these shortcomings, we introduce rSDE-Bench, which includes measurable and diverse requirements in the task description, and provide a matched evaluation of how well these requirements are fulfilled at the functional level to provide more practical and accurate assessments of development effectiveness.




% ##################### 10.1 1:00 ###################

 
% \noindent\textbf{Software development benchmarks.} Software development is a user-requirement-oriented, systematic, and complex task that often requires team collaboration to produce a fully functional product.~\cite{software_survey2024} Given this complexity, it is essential for software development benchmarks to clearly define the tasks involved and establish methods to evaluate how effectively these tasks are completed. Existing benchmarks can be categorized into three types:
% 1) Function-level completion tasks (e.g., HumanEval~\cite{humaneval2021}, MBPP~\cite{mbpp2021}, CodeContests);
% 2) Software generation tasks (e.g., SRDD~\cite{chatdev2023}, SoftwareDev~\cite{metagpt2023});
% 3) Bug repair tasks (e.g., SWE-bench~\cite{swebench2023} for github issues).
% However, these benchmarks do not evaluate models' software development capabilities from the perspective of user requirements, which are fundamental to the entire development process. Requirements define the functions and features a software system should have, describing both its external behavior and internal attributes, and providing clear goals for subsequent design and implementation.
% For example, SoftwareDev~\cite{metagpt2023} lacks precise task definitions and relies on semantic metrics like similarity, which are insufficient for assessing the actual effectiveness of software development. To address these shortcomings, we introduce rSDE-Bench, which defines tasks based on the core of software development, user requirements, and uses function-based checks aligned with these requirements for more practical and accurate evaluation.

% CodeContests好像没有对应的paper



% 软件开发是一个面向用户需求、系统且复杂的工作，实际中一个完善的软件往往需要一个团队的合作来开发。因此有很多多智能体的工作将软件开发纳入考量，并构建了一些软件开发的benchmark。这些benchmark包含了关于任务的定义以及评估标准，但这些benchmark对任务缺乏明确的定义，且评估方式也不合理，不能正确反应软件开发的关键因素：需求的完成情况。在这里我们对这个任务有关的benchmark进行了分类。

% Original version from Dr. Hu
% \noindent\textbf{Software development benchmarks.} Software development benchmarks aim to evaluate models in the task of synthesizing code from natural language descriptions. These benchmarks can test generation, and reasoning capabilities, and have long been used as key indicators for measuring the performance of language models. Existing benchmarks for software development can mainly be classified into three categories: i) function level completion tasks (e.g., HumanEval, MBPP, Contest); ii) software generation tasks (e.g., SRDD, MetaGPT); and iii) bug repair tasks (e.g., SWE-bench). However, these benchmarks either lack diverse software definitions or fail to incorporate requirement-aware measurement. To address these shortcomings, we introduce **, which aims to fill this gap by **.



==> EvoMAC/content/03-benchmark.tex <==
\vspace{-4mm}
\section{rSDE-Bench: requirement-Oriented Software Development Engineering Benchmark}
\vspace{-2mm}

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=1.0\linewidth]{figures/requirement.pdf}
%     \vspace{-6mm}
%     \caption{Comparison of instruction-oriented and requirement-oriented (rSDE-Bench) benchmarks in evaluating the website DailyHealthTips.}
%     % \caption{Here is an example of an website software requirement instance in our rSDE-Bench, a test case , and the test reports.}
%     \label{fig:requirement}
%     \vspace{-6mm}
% \end{figure}

% In the complex landscape of software development, the necessity for precise software requirements is crucial. \Note{sc: confusing, can you compare with the current benchmark?} These requirements elucidate each functionality and constraint of the software, item by item. They serve as the quantifiable benchmarks against which the efficacy of the developed software can be measured. They serve as the measurable standards that enable a detailed, itemized assessment of whether the developed software has achieved its intended objectives.
% Benchmarks~\cite{humaneval2021,mbpp2021} for evaluating the code generation capabilities of models initially focused on function-level tasks, where models have now demonstrated considerable success. As a result, researchers have begun exploring more complex tasks involving full software development to better assess the models’ capabilities in generating code. In these newer benchmarks~\cite{chatdev2023}, models are typically prompted by relatively simple instructions to generate entire software projects. However, these methods often lack the specificity required to assess how well the generated software aligns with the given instructions, making the evaluation less clear.

% To address these gap, we introduce
This section introduces \texttt{rSDE-Bench}, a requirement-oriented benchmark designed to assess the ability of models to handle software-level coding tasks. Each coding task involves multiple detailed software requirements. These requirements specify each functionality and constraint of the software, item by item, serving as measurable benchmarks for assessing the software’s effectiveness.
% They serve as the quantifiable benchmarks against which the efficacy of the developed software can be measured. They provide measurable standards that enable a detailed, itemized assessment of whether the developed software has achieved its intended objectives.
As shown in Fig.~\ref{fig:evalation}, unlike previous instruction-oriented approaches~\cite{chatdev2023,metagpt2023} which rely on brief instructions as input, \texttt{rSDE-Bench} uses comprehensive software requirements as input, complemented by unit test cases to automatically evaluate the correctness. This benchmark provides software-level coding tasks and automatic evaluation, aligning more closely with real-world software development practices.
% This approach provides a more objective and precise assessment of how well models fulfill the specified requirements, aligning more closely with real-world software development practices.
% \Note{sc: overview of what?}

% Inspired by the clarity and precision of software requirements, we introduce a novel benchmark designed to evaluate the capabilities of models in generating software code, which is called \texttt{rSDE-Bench}; see Fig.~\ref{fig:requirement}. 
% Contrasting with previous evalation methods, which rely on brief instructions to drive model, rSDE-Bench is requirement-oriented leveraging detailed software requirements as input. 
% Aditionally, it enables a more accurate and quantifiable assessment of the generated code's effectiveness, and is also closer to real software development process. 

\vspace{-4mm}
\subsection{Benchmark construction}
\label{Benchmark:construction} 
\vspace{-2mm}

% \Note{sc: what games? what websites? difficulty }

% rSDE-Bench provides a comprehensive framework for evaluating the code generation capabilities of models, focusing on two software categories: game and website. These categories are chosen due to their inherent complexity and structural differences, which reflect the challenges of real-world software development. The diverse distribution of test cases, as shown in Fig~\ref{Fig:testcase_dist}, further highlights the distinct characteristics of each category, covering key aspects such as user management, page display, logic, and game operations. As shown in Table~\ref{Table:benchmark_stat}, the benchmark includes 53 unique software requirements and approximately 700 test cases, ensuring broad coverage across both domains. Each task is specifically designed to align with a given requirement, providing an accurate and objective assessment of the generated code. The use of unit tests, with clearly defined inputs and expected outputs, ensures a rigorous and quantifiable evaluation of model performance. To create high-quality software requirements and corresponding test cases, we use a two-step process.Please refer to App.~\ref{app:benchmark} for details.

rSDE-Bench involves two typical real-world software types: game and website. They can reflect different coding capacities demanded in realistic software development.
% They are chosen for their complexity and structural differences.
% \Note{sc: what is the difference} which mirror real-world development challenges. 
Game often requires handling dynamic interactions, real-time state changes, and user-driven operations, focusing on elements like logic execution, initialization, and game state transitions. Website emphasizes static and dynamic content management, user interaction through forms and buttons, and ensuring page elements are displayed and functional. 
% These structural differences mirror the challenges of real-world development, where diverse requirements demand different coding skills.
rSDE-Bench involves diverse requirements, each paired with a test case. Specifically, rSDE-Bench provides 53 unique coding tasks and 616 test cases. For details on the benchmark construction, software statistics, software requirements, and test case examples, see Sec.~\ref{app:benchmark} in the Appendix.

rSDE-Bench introduces two requirement difficulty levels, including basic and advanced, to reflect the varying complexity of real-world software development tasks. The basics reflect the fundamental and more achievable requirements, such as interaction, control, and logging. The advanced reflects more complex software functionalities, such as game logical rules, and dynamic web content management. The details can be referred to the appendix.



\vspace{-2mm}
\subsection{Automatic Evaluation}
\vspace{-2mm}

\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/evaluation.pdf}
    \vspace{-6mm}
    \caption{Comparison between instruction-oriented and requirement-oriented evaluations. rSDE-Bench accurately reflects requirement fulfillment with the proposed accuracy score of $2/13$, while the indrection evaluation misjudges with high scores ($0.89$), failing to detect missing functionality.}
    \vspace{-4mm}
    \label{fig:evalation}
\end{figure}

rSDE-Bench supports automatic evaluation of requirement correctness.
It achieves this by pairing a specifically designed black-box test case with each requirement. The test case can directly verify whether the generated code achieved the requirement.
Its evaluation metric is the accuracy, which quantifies the proportion of correctly passed test cases. It is similar to the \texttt{pass@1} metric in HumanEval~\cite{humaneval2021}, which evaluates the pass ratio of correctly achieved functions against the total functions via unit test verification. 
It is a fully automated evaluation process, eliminating the need for human involvement while still providing accurate and reliable assessments.

% ensuring a clear measure of whether the model's output satisfies the required functionality and constraints. We use black-box testing to simulate interactions between humans and the software, verifying whether each requirement is correctly implemented.

% It uses accuracy as an evaluation metric, which quantifies the proportion of correctly passed test cases. It is similar to the \texttt{pass@1} metric in HumanEval~\cite{humaneval2021}, which evaluates the pass ratio of correctly achieved functions against the total functions via unit test verification.  It is a fully automated evaluation process: generated code can be automatically tested, eliminating the need for human involvement while still providing accurate and reliable assessments.
% \Note{sc: highlight how it is automatic}

% Fig.~\ref{fig:requirement} shows the evaluation methods of instruction-oriented benchmarks compared to \texttt{rSDE-Bench}. 
Previous benchmarks for software code generation mainly rely on two evaluation methods. One method is human evaluation~\cite{metagpt2023}, which is time-consuming and not scalable for large datasets.
The other method is indirect evaluations~\cite{chatdev2023}, which defines metrics like consistency, completeness, and quality. Consistency measures how closely the generated software aligns with the original requirement description by comparing the cosine similarity between the two. Completeness is determined by detecting the presence of placeholder (such as \texttt{pass} or \texttt{TODO}), which results in a binary value of 0 or 1. Quality is then calculated as the product of several factors: consistency, completeness, and executability.
As illustrated in Fig.~\ref{fig:evalation}, they could not measure the correctness of the generated code in fulfilling requirements. 
% \Note{sc: still lack of an example}  
% For instance, , indirect evaluation incorrectly assesses completeness as 0 due to the pass statement in the generated code, even though it is not an actual placeholder. This results in a quality score of 0, which fails to reflect the true state of the generated code.
In contrast, \texttt{rSDE-Bench}'s test cases-based evaluation is more rigorous and precise. These test cases can accurately verify the correctness of generated code in fulfilling the requirements.
\texttt{rSDE-Bench} promises reliable and scalable automatic evaluation. In the experiments, we have validated the significant advantages of the proposed automatic evaluation over the previous metrics, including consistency and quality; see Fig.~\ref{Table:humanevalpercentage}.

% By designing test cases based on specific software requirements and using black-box testing, we can directly and objectively evaluate how well the generated code

\vspace{-2mm}
\subsection{Features}
\label{Benchmark:features}
\vspace{-2mm}

% \noindent\textbf{Challenging and diverse software requirements.} Software development requirements in rSDE-Bench are typically long-form text (averaging 507/1011 words for game and website benchmarks, respectively). Unlike existing instruction-oriented benchmarks~\cite{humaneval2021,mbpp2021,swebench2023}, which focus on brief instructions, rSDE-Bench involves more challenging and varied requirements, closely reflecting the challenges of real-world software development. This approach not only enhances the evaluation of code generation models, but also allows for a more thorough assessment of the current models' ability to handle realistic software demands, providing a clearer view of their practical coding capabilities.

\noindent\textbf{Challenging and diverse software requirements.} rSDE-Bench features long-context software requirements (averaging 507/1011 words for game and website tasks, respectively), unlike instruction-oriented benchmarks~\cite{humaneval2021,mbpp2021,swebench2023} that rely on brief prompts. These detailed requirements better reflect real-world lengthy and complex software development challenges.
% , allowing for a more thorough assessment of models' ability to handle practical .

\noindent\textbf{Requirement-aware precise and efficient evaluation.} 
rSDE-Bench employs detailed software requirements and automated unit tests to precisely measure how well generated software meets its objectives. Generated codes are evaluated based on pass rates from running specific test cases, offering an accurate and efficient process. In contrast, instruction-oriented benchmarks rely on brief prompts, which lack constraints and make evaluation less reliable, often requiring labor-intensive or indirect evaluation.

% rSDE-Bench employs detailed software requirements and unit test cases to directly and precisely measure how well the generated software meets its objectives, offering a more accurate and efficient evaluation process. Each of our task is automatically evaluated based on the pass rate of the requirements via running specific test cases. In comparison, exiting software development are mainly instruction-oriented, relying on brief and generalized instructions to prompt code generation. This approach creates two major challenges: first, the brevity of the instructions provides insufficient constraints on the generated software, making it difficult to evaluate how well the output aligns with the intended goals. Second, the evaluation methods used, such as human evaluation or code indirect evaluation, are labor-intensive or lack precision.

% \noindent\textbf{Driving advancements in software code generation.}
% rSDE-Bench can accelerate progress in automated software generation by introducing challenges that closely mimic real-world development tasks by introducing multiple layers of complexity. First, it pushes models to generate large, multi-file, project-level codebases, a crucial step toward building fully functional software systems. Second, it requires models to interpret and implement detailed, long-form software requirements, promoting deeper understanding and precision in code generation. Third, it assesses robustness in managing long-context scenarios, where the model must integrate and maintain consistency across multiple code segments. This comprehensive approach challenges the model’s ability to handle full-spectrum software development tasks—skills like requirement analysis, multi-step reasoning, and long-context code generation. By addressing these essential aspects of software development, rSDE-Bench lays the foundation for more capable, autonomous systems that can handle increasingly complex software generation tasks, pushing the boundaries of what is possible in the field.

==> EvoMAC/content/03-benchmark_old.tex <==
\section{RSD-Bench: Requirement-Oriented Software Development Benchmark}

% This section presents~\texttt{RSD-Bench}, a benchmark that targets to evaluate models on the task of generating codes to complete the software development requirements. To achieve comprehensive and objective evaluation, RSD-Bench features two typical realistic software types: game and website, and quantitative requirement-aware evaluation metrics. 
% The task formulation, benchmark construction, and features are introduced in the following Sec.~\ref{Benchmark:formulation},~\ref{Benchmark:construction}, and~\ref{Benchmark:features}. 
Generating code that precisely matches the defined software requirements is the cornerstone of a software development project. Therefore, to evaluate the capability of models to generate code that satisfies well-defined software requirements, we meticulously craft a benchmark~\texttt{RSD-Bench}. It encompasses the software requirements for two quintessential types of real-world software: games and websites. Additionally, it provides a rigorous and quantitative requirement-aware evaluation metrics for measuring how effectively generated code meets its intended objectives, thus aligning with the intricate demands of software engineering.


\begin{minipage}{0.4\textwidth}
% \begin{table}[]
\centering
\scalebox{0.65}{
\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{Benchmark} & \multicolumn{2}{c}{Software} & \multicolumn{2}{c}{Test Case} \\
                           & Amount   & Length  & Basic        & Advanced        \\ \midrule
Website                    & 45       &         1011/1553           &        292      &         247        \\ 
Game                       & 8        &         507/788           &        46      &         31        \\
\bottomrule
\end{tabular}}
\captionof{table}{Benchmark statistics}
\label{Table:benchmark_stat}
% \end{table}
\end{minipage}
\begin{minipage}{0.6\textwidth}
% \begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/combined_test_cases_with_format.pdf}
    % \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
    \captionof{figure}{Test case statistics of Game and Website tasks.}
    \label{Fig:testcase_dist}
% \end{figure}
\end{minipage}



\subsection{Benchmark construction}
\label{Benchmark:construction}

RSD-Bench includes two typical, real-world software types: games and websites, see Table.~\ref{Table:benchmark_stat}. The website benchmark is semi-automatically generated and scalable for large-scale expansion. The game benchmark is manually constructed, as each game has unique running rules, and its GUI is difficult to quantify, requiring human input to define measurable requirements. Both benchmarks follow a common two-step process to create high-quality task instances. After generating the task instances, we manually remove any unclear or unstable ones to ensure the benchmark's stability and measurability.

\noindent\textbf{Step 1: Software requirement generation.} Each task instance begins by generating clear and measurable software requirements. For the game benchmark, we focus on common real-world games and document detailed task requirements, including GUI layout initialization, interaction methods, expected game states, and game state logging. In addition to the game rules, we include game state logging as a requirement for automatic evaluation of the task. For the website benchmark, we start with a brief requirement that outlines the website’s workflow and then use large models to enrich the details following a predefined pattern. This approach ensures efficiency and scalability for the website benchmark.

\noindent\textbf{Step 2: Requirement-based test cases generation.} 
Each task instance incorporates black-box test cases to quantitatively evaluate the fulfillment of the generated software requirements. For the game benchmark, we manually create test cases, similar to the HumanEval~\cite{humaneval2021} code completion benchmark, which checks state changes based on specific inputs. In the game context, we assess game state changes in response to specific GUI interactions. For the website benchmark, large models are used to generate test cases based on the software requirements, followed by manual corrections to clarify any ambiguous cases.

\subsection{Benchmark formulation}
\label{Benchmark:formulation}

% The task is defined as generating codes to complete the software development requirements. Each task instance includes pairwise natural language-specified software requirements and associated test cases to evaluate the requirement completeness of the generated code.
% The task goal is to generate code given the natural language specified software requirement. Its input is the software requirement, and the evaluation is .


\noindent\textbf{Requirement-based model input.} A model is provided with clear and comprehensive software requirements. As depicted in Fig.~\ref{}, they are specified with natural language, which defines the software's targeted features and detailed workflows, rules, and states, such as interaction types and expected effects. These requirements are categorized into two levels of difficulty: basic and advanced, tailored to the complexity of each specific requirement. 
% We define two types of requirements: basic and advanced. 
% , RSD-bench designs software requirements for two types of software development tasks: games and websites. 
The basic requirements reflect the most fundamental capabilities, including software setup, keyboard control, clicking, and logging. The advanced requirements reflect more complex capabilities, including logical rules, and compositional effects. The model takes the software requirements as input to generate code. 

\noindent\textbf{Requirement-based evaluation metrics.} 
To evaluate the requirement completeness of the generated code, we associate black-box test cases (cf. Sec~\ref{Benchmark:construction}) with each defined software requirement. If the generated code can pass the test case, we consider the corresponding requirements are successfully achieved. The metric is the ratio of the passed test cases.

\subsection{Features}
\label{Benchmark:features}

\noindent\textbf{Complex and diverse software requirements.} Software development requirements in RSD-bench are typically long (averaging 507/1011 words for game and website benchmarks, respectively). Unlike existing function-level code completion and bug-fixing benchmarks, which focus on specific functions or issues, RSD-bench involves more complex and varied requirements, making it closer to real-world software development projects.

\noindent\textbf{Requirement-aware automatic evaluation.} Each task is automatically evaluated based on the pass rate of the requirements via running test cases. Existing software development benchmarks often define vague or unmeasurable requirements, relying on human evaluation or the similarity between generated code and requirements. These methods lack scalability and provide imprecise software performance evaluation. RSD-bench offers automatic, direct measurement of how well a task's software development goals are met.

\noindent\textbf{New and realistic software development challenges.} Solving tasks in RSD-bench demands: i) generating large codebases, ii) analyzing the fulfillment of each requirement, and iii) integrating code within a long context. This challenge requires advanced skills and knowledge typical of experienced software engineers, which are not commonly tested in traditional code generation benchmarks. These capabilities includes requirement analysis, task decomposition, code generation, testing, bug localization, and bug fixing.



==> EvoMAC/content/04-system.tex <==
\vspace{-4mm}
\section{EvoMAC: Self-Evolving Multi-Agent Collaboration Network}
\vspace{-2mm}

This section presents~\texttt{EvoMAC}, a novel self-evolving multi-agent collaboration network and its application to software development. The key feature of~\texttt{EvoMAC} is its ability to iteratively adapt both agents and their connections during test-time for each task, mimicking the back-propagation process, a core algorithm in neural network training. We first formulate a general self-evolving paradigm in Sec.~\ref{System:framework} and then describe its application to software development in Sec.~\ref{System:evolving}. 
% The procedure includes three key elements: forward pass, loss computation, and textual back-propagation.

\vspace{-2mm}
\subsection{A general self-evolving paradigm via textual backpropagation}\label{System:framework}
\vspace{-2mm}

\noindent\textbf{Multi-agent collaboration network.} A multi-agent collaboration (MAC) network is a computational graph representing agentic workflows, where multiple agents empowered by LLMs interact as interconnected nodes to coordinate and share information for complex task-solving. The intuition behind to divide the complex task into more specific and manageable subtasks for each agent, allowing the overall task to be gradually conquered through the agentic workflow. Mathematically, we represent a MAC network with $N$ autonomous agents as a directed acyclic graph $\mathcal{A} = (\mathcal{V}, \mathcal{E})$, where $\mathcal{V} = \{v_i\}_{i=1}^{N}$ is the set of $N$ nodes, and $\mathcal{E} = \{e_{i,j}\}_{i,j \in [1, \dots, N], i \neq j}$ is the set of directed edges with no circles. The $i$-th node $v_{i}$ represents the $i$-th autonomous agent with the prompt $p_{i}$, which specifies its subtask. The edge $e_{i,j}$ represents the task dependency between the $i$-th agent and the $j$-th agent, indicating that the $j$-th agent's subtask should be executed after the $i$-th agent's subtask in the agentic workflow. The overall graph topology specifies the agentic workflow. Analogy to traditional neural networks, agents function similarly to neurons, with agent prompts serving as neurons' weights and the agentic workflow as the layers and connections. 


The feed-forward pass of MAC network is the execution of the agentic workflow. In this process, each agent is given two inputs: the initial task requirement and the output from the previous agent. Using these, each agent produces an output that fulfills its specific subtask. Eventually, the last agent's generation constitutes the final output, integrating all completed subtasks. Note that the initial task requirement is input to each agent as context, providing supplementary details to aid in the implementation of each subtask.


% processes the task requirements through the MAC network and gathers the generated output, denoted as $\mathbf{G}^{(k)} = \Phi(\mathbf{X}, \mathcal{A}_g^{(k)})$, where $k$ denotes the evolving time. During this stage, given the computational graph $\mathcal{A}_c^{(n)}=\{\mathcal{V}_c^{(n)},\mathcal{E}_c^{(n)}\}$, its directed edges $\mathcal{E}_c^{(n)}$ decide the topological order of the $K$ agents, dictating the sequence of the agentic workflow. This sequence is denoted as $\mathcal{I}_c^{(n)}=[ \ldots i, j,\ldots,m]$, where each element represents the agent index, and the overall length is $K$, the same as the agent amount. Following this sequence, each agent receives the input text and the generated output of the previous agent, refining the generation based on prompts through role-playing. Specifically, the execution of the $j$-th agent, following the $i$-th agent whose output is $o^{(n)}_{c,i}$, is expressed as $o_{c,j}^{(n)}=\rho(\mathcal{X},o_{c,i}^{(n)},p_{c,j}^{(n)})$, where the role-playing function is represented by $\rho(\cdot)$. Ultimately, the output from the final agent forms the overall final generation, this is, $\mathcal{Y}^{(n)}=o_{c,m}^{(n)}$.\Note{sc: it seems this should be illustrated in the beginning of section 3.1}

Recently, various MAC networks have been designed using human expertise to assign fixed agent prompts and workflows~\cite{metagpt2023, chanchateval}, resembling untrained neural networks. However, these designs solely rely on human priors and lack adaptability, causing limited performance improvement over a single agent. To overcome this, inspired by neural network training, we propose a self-evolving paradigm for multi-agent collaboration networks, enabling both agents and their connections to dynamically evolve during test-time for each given task.

% The key idea behind enabling the self-evolving paradigm is to introduce an accurate assessment of the gap between the current MAC network's output and the target, providing guidance for the network's improvement.

% To achieve this, we formulate an optimization problem analogous to supervised learning in traditional neural network training. 

% and offers informative cues to guide the MAC network 


\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/Framework.png}
    \vspace{-6mm}
    \caption{The general self-evolving paradigm.}
    \label{fig:framework}
    \vspace{-6mm}
\end{figure}

\noindent\textbf{Optimization problem.}
Here we consider a general generation task. During test-time, given a task, the MAC network performs a feed-forward pass to generate the final output without knowing its quality. The key to evolution during test-time is to set up a target proxy for the MAC network to guide its improvements in the generated output. Here we consider this target proxy as the conditions for task completion, such as unit tests in coding, and we can produce such a target proxy by another group of autonomous agents based on the same task description. Then, the quality of each generated output can be verified according to the target proxy. This approach relies on two key assumptions: (i) generating a target proxy is significantly simpler than completing the original generation task, and (ii) the generated output can be correctly verified against the target proxy through an objective environment. These assumptions are practical in many applications. For example, in code generation, producing unit tests, the expected input-output pairs, is much easier than generating the entire code; meanwhile, a code compiler naturally acts as the objective environment to check the correctness of the generated code against the unit test, providing objective and informative feedback.

Mathematically, let $\mathbf{X}$ be the textual description of a task. Given the MAC network $\mathcal{A}_g$, the generated output is $\mathbf{G} = \Phi(\mathbf{X}, \mathcal{A}_g)$, where  $\Phi(\cdot, \cdot)$ is the general feed-forward operator that executes the agentic workflow, processing the input text through the MAC network. Similarly, the target proxy is $\mathbf{T} = \Phi(\mathbf{X}, \mathcal{A}_t)$, where $\mathcal{A}_t$ is another MAC network designed for producing the target proxy. Note that we aim to evolve and optimize $\mathcal{A}_g$, while keep $\mathcal{A}_t$ predefined and fixed. The optimization of our self-evolution is formulated as, 
\begin{equation}
\label{eq:optimization}
     \mathcal{A}_g^{*} = \underset{\mathcal{A}_g}{\min}~\langle \Phi(\mathbf{X}, \mathcal{A}_g), \mathbf{T}\rangle_{E}, ~~\text{subject~to:}~~ \mathbf{T}=\Phi\left(\mathbf{X}, \mathcal{A}_t \right),
\end{equation}
where $\langle \cdot,\cdot\rangle_{E}$ is an objective environment executor that receives the generated output and the target proxy as inputs and outputs a text-based environmental feedback.  Akin to the loss function in traditional neural network training, which quantifies the difference between the generated output and the ground-truth, the objective in~\eqref{eq:optimization} evaluates whether the generated output meets the conditions of the task completion using the environment, subsequently producing execution reports as the text-based environmental feedback. Here the minimization operation $\min$ is defined to reduce the failures during execution. With the guidance of the target proxy and the objective feedback given by the environment, the MAC network can improve its success rate of task completion during test time. 

Note that, another straightforward way to enable the MAC network's evolution is through the self-critique strategy~\cite{symbolic2024,Valmeekam2023CanLL,Xu2024ChatGLMMathIM,Asai2023SelfRAGLT}, which employs a critique agent to assess the generated output directly. This approach has two inherent limitations: i) the critique may be subjective and biased, and ii) the critique agent can have hallucinations, causing inconsistencies and errors. These limitations can cause the MAC network to become entrenched in its own preferences or evolve in the wrong direction, especially iterating multiple times; see our experimental validations in Tab.~\ref{Table:ablation study}. In comparison, our approach leverages an environment executor to provide objective feedback, preventing bias and hallucinations.

While we use the analogy between our self-evolution process and neural network training for motivating, they are significantly different in three key aspects: (i) our self-evolution occurs at test time without a dedicated training phase; (ii) it evolves for each specific task individually rather than over a batch of samples; and (iii) the environmental feedback are usually texts, not be numerical values, which cannot be optimized by the standard backpropagation. This motivates us to propose our textual backpropagation.


\noindent\textbf{Solution based on textual backpropagation.} The self-evolution solution iteratively updates the MAC network using a textual backpropagation algorithm, guided by the environmental feedback. The core idea is to analyze the influence of each agent in the MAC network $\mathcal{A}_g$ to the final environmental feedback and use these analyses to update the agent prompts and the agentic workflow in $\mathcal{A}_g$. This is achieved by two collaborative agents, each responsible for one of the two key steps: (i) textual gradient analysis and (ii) network update. The overall algorithm can refer to Alg.~\ref{alg:EvoMAC} in the appendix.

First, the gradient agent takes the environmental feedback as the input and outputs textual gradients that describe the impact of each agent in the MAC network. Let $\mathcal{A}_g^{(k)}$ and $\mathbf{L}^{(k)}$ be the MAC network and  the environment feedback at the $k$-th iteration. The textual gradient is then $\nabla \mathbf{L}^{(k)} = \mathcal{G}(\mathcal{A}_g^{(k)},\mathbf{L}^{(k)})$, where $\mathcal{G}(\cdot,\cdot)$ is the gradient analysis operator managed by the gradient agent; see its prompt in Appendix. The textual gradient details three-fold information for each agent inside $\mathcal{A}_g^{(k)}$: 1) whether this agent's subtask is fulfilled; 2) whether this agent introduces errors; and 3) whether any subtask is missed in the current MAC network.

Second, based on the textual gradients, the updating agent iterates the MAC network as $\mathcal{A}_g^{(k+1)} = \mathcal{U}(\mathcal{A}_g^{(k)}, \nabla \mathbf{L}^{(k)})$, where $\mathcal{U}(\cdot,\cdot)$ is the updating operator managed by the updating agent. This operator guides the updates from three-folds: 1) removing the agents whose subtasks have been completed; 2) revising the erroneous agent's prompts by adding potential solutions provided in the gradient analysis; and 3) adding new agents for missing subtasks and restructuring the workflows based on the subtask dependencies noted in the gradient analysis; see the prompt details in Appendix. These adjustments address existing issues and fulfill unmet requirements in the current generation of the MAC network, promising improvements in the updated version. 



% \noindent
% \begin{wrapfigure}{r}{0.5\textwidth}
% \begin{algorithm}[H]
% \footnotesize
% \caption{\footnotesize{Multi-Agent Evolving Paradigm}}
% \SetAlgoLined
% \KwIn{$\mathbf{X}$ \Comment{Task input}, $\mathcal{A}_{g}^{(0)}$ \Comment{Initialized MAC network}, $\mathcal{A}_{t}$ \Comment{Designed MAC network to generate target proxy}, $\mathcal{G}$ \Comment{Agent-based gradient function}, $\mathcal{U}$ \Comment{Agent-based update function}, $E$ \Comment{Environment tool to generate loss}}
% Define $K$ as iteration time, $\Phi$ as forward operator\;
% \textcolor{blue}{\#~Simulated Target}\;
% $\mathbf{T} = \Phi(\mathbf{X},\mathcal{A}_{t})$\;
% \textcolor{blue}{\#~Evolving Procedure}\;
% \For{$k = 0, 1, \dots, K-1$}{
%     \textcolor{blue}{\#~Forward Pass}\;
%     $\mathbf{G}^{(k)} = \Phi(\mathbf{X}, \mathcal{A}_g^{(k)})$;             
%     \hspace{1.3cm}\Comment{\footnotesize{Generation}}\;
%     \textcolor{blue}{\#~Loss Computation}\;
%     $\mathbf{L}^{(k)}=\langle \mathbf{G}^{(k)}, \mathbf{T}\rangle_{E}$;\hfill \hfill \hfill \hspace{0.9cm}\Comment{\footnotesize{Env Feedback}}\;
%     \textcolor{blue}{\#~Textual Backpropagation}\;
%     $\nabla \mathbf{L}^{(k)} = \mathcal{G}( \mathcal{A}_g^{(k)}, \mathbf{L}^{(k)})$;
%     \hspace{0.1cm}\hfill \Comment{\footnotesize{Textual gradient}}\;
%     $\mathcal{A}_g^{(k+1)} = \mathcal{U}(\mathcal{A}_g^{(k)}, \nabla \mathbf{L}^{(k)})$;
%     \hspace{0cm}\hfill \Comment{\footnotesize{Update agents}}\;
% }
% \Return $\mathcal{A}_g^{(K)}, \mathbf{G}^{(K)}$\;
% \end{algorithm}
% \end{wrapfigure}

Note that, the key of the textual backpropagation is the prompt designs for both gradient analysis and network updates. The design must i) thoroughly evaluate the subtask of each agent in the MAC network according to the objective environment feedback and determine necessary adjustments to the MAC network to address existing issues, fulfilling the unmet requirements; and ii) maintain coherence, ensuring that issues identified by the gradient agent can be effectively resolved by the updating agent's modifications to the MAC network.





% \begin{algorithm}[!t]
%     \small
%     \setlength{\intextsep}{0pt} 
% 	\caption{Multi-Agent Evolving Framework} 
% 	\begin{algorithmic}[1]
%         \Require $\mathbf{X}$ \Comment{Task input}, $\mathcal{A}_{g}^{(0)}$ \Comment{Initialized MAC network}, $\mathcal{A}_{t}$ \Comment{Designed MAC network to generate target proxy}, $\mathcal{G}$ \Comment{Agent-based gradient function}, $\mathcal{U}$ \Comment{Agent-based update function}, $E$ \Comment{Environment tool to generate loss}
%         \State Define $K$ as the number of self-evolving iterations, $\Phi$ as MACN generation process
%         \State {\color{blue} \#~Simulated Target}
%         \State $\widehat{\mathbf{T}} = \Phi(\mathbf{X},\mathcal{A}_{t})$ 
%         \State {\color{blue} \#~Evolving Procedure}
%         \For {$k = 0, 1, \dots, K-1$}
%             \State {\color{blue} \#~Forward Pass}
%             \State $\mathbf{G}^{(k)} = \Phi(\mathbf{X}, \mathcal{A}_g^{(k)})$
%             \State {\color{blue} \#~Loss Computation}
%             \State $\mathbf{L}^{(k)}=\langle \mathbf{G}^{(k)}, \mathbf{T}\rangle_{E}$ \Comment{Use environment feedback as textual loss}
%             \State {\color{blue} \#~Textual Backpropagation}
%             \State $\nabla \mathbf{L}^{(k)} = \mathcal{G}(\mathbf{L}^{(k)},\mathcal{A}_g^{(k)})$ \Comment{Summarize textual gradient}
%             \State $\mathcal{A}_g^{(k+1)} = \mathcal{U}(\mathcal{A}_g^{(k)}, \nabla \mathbf{L}^{(k)})$ \Comment{Update agent prompts and pipeline}
%         \EndFor
%         \State \Return $\mathcal{A}_g^{(K)}, \mathbf{G}^{(K)}$
% 	\end{algorithmic}
% 	\label{alg:EvoMAC}
% \end{algorithm}

% \begin{algorithm}[!t]
% 	\caption{Multi-Agent Evolving Framework} 
% 	\begin{algorithmic}[1]
%         \Require $\mathbf{X}$ \Comment{Task input}
%         \Require $\mathcal{A}_{g}^{(0)}$ \Comment{Initialized MAC network: agent prompts and pipeline}
%         \Require $\mathcal{A}_{t}$ \Comment{Designed MAC network to generate target proxy}
%         \Require $\mathcal{G}$ \Comment{Agent-based gradient function}
%         \Require $\mathcal{U}$ \Comment{Agent-based update function}
%         \Require $E$ \Comment{Environment tool to generate loss}
%         \State Define $K$ as the number of self-evolving iterations, $\Phi$ as MACN generation process
%         \State {\color{blue} \#~Simulated Target}
%         \State $\widehat{\mathbf{T}} = \Phi(\mathbf{X},\mathcal{A}_{t})$ 
%         \State {\color{blue} \#~Evolving Procedure}
%         \For {$k = 0, 1, \dots, K-1$}
%             \State {\color{blue} \#~Forward Pass}
%             \State $\mathbf{G}^{(k)} = \Phi(\mathbf{X}, \mathcal{A}_g^{(k)})$
%             \State {\color{blue} \#~Loss Computation}
%             \State $\mathbf{L}^{(k)}=\langle \mathbf{G}^{(k)}, \mathbf{T}\rangle_{E}$ \Comment{Use environment feedback as textual loss}
%             % \State $\mathcal{F}^{(n)} = \mathcal{L}(\mathcal{Y}^{(n)},\widehat{\mathcal{Y}})$ \Comment{Use environment feedback as textual loss}
%             \State {\color{blue} \#~Textual Backpropagation}
%             \State $\nabla \mathbf{L}^{(k)} = \mathcal{G}(\mathbf{L}^{(k)},\mathcal{A}_g^{(k)})$ \Comment{Summarize textual gradient}
%             \State $\mathcal{A}_g^{(k+1)} = \mathcal{U}(\mathcal{A}_g^{(k)}, \nabla \mathbf{L}^{(k)})$ \Comment{Update agent prompts and pipeline}
%         \EndFor
%         \State \Return $\mathcal{A}_g^{(K)}, \mathbf{G}^{(K)}$
% 	\end{algorithmic}
% 	\label{alg:EvoMAC}
% \end{algorithm}



\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/System.png}
    \vspace{-6mm}
    \caption{EvoMAC takes task requirements as input and iteratively updates the coding team to generate code that better fulfills the requirements.}
    \label{fig:system}
    \vspace{-6mm}
\end{figure}

\vspace{-2mm}
\subsection{Self-evolution for software development}
\label{System:evolving}
\vspace{-2mm}

In this section, we apply the self-evolving paradigm to the task of software development. The overall architecture of the proposed self-evolving multi-agent collaboration network for software development is illustrated in Fig.~\ref{fig:framework}. Given a coding task, the coding team, corresponding to the MAC network $\mathcal{A}_g$, generates all the codes through its forward-pass; the testing team, associated with the MAC network $\mathcal{A}_t$, is responsible for creating the target proxy; that is, unit tests of the coding task; and the objective environment tool is realized through the compiler. The identified bugs during execution form the textual environmental feedback. The updating team, consisting of two collaborative agents, manages the textual backpropagation. By continuously cycling through feed-forward, feedback collection, and textual backpropagation processes, the coding team is iteratively refined to more closely align with the test cases. The detailed implementation of agents can refer to Sec.~\ref{app:prompts} in the Appendix.

Since unit test generation is much easier than the original logical code generation, the testing team usually can produce high-quality test cases, which are closely aligned with the task requirements. Then, improving alignment with the unit tests through MAC network updates ensures better adherence to the actual task requirements.


\noindent\textbf{Coding team for feed-forward.} In the feed-forward process, the coding team synthesizes code according to the given coding task. To handle the extensive software requirements, the coding team is implemented as a MAC network. It divides the comprehensive requirements into a sequence of smaller, more specific function implementation subtasks, and progressively conquers them through the agentic workflow. 
Unlike existing MAC systems that heuristically decompose coding tasks and define the agentic workflow, we initialize the MAC network using a novel self-organizing approach.
A coding organizer agent automatically and flexibly decomposes the task requirements into subtasks and assembles the coding agent team accordingly. The number of coding agents is dynamic, adjusting in response to the task requirements. Note that, the quality of the generated code is unknown during the forward pass, which necessitates the self-evolving paradigm to iteratively refine the generation.

\noindent\textbf{Testing team and compiler for feedback collection.} 
To verify whether the generated code meets the requirements of the coding task, we employ unit tests as the target proxy. These test cases consist of input-output pairs tailored to specific requirements. For example, a test case for a keyboard control requirement would detail the type of control as the input and describe the expected behavior as the output. To create flexible and comprehensive unit tests, we set up the testing team as a MAC network and also initialize it in a self-organized way. A testing organizer agent automatically decomposes our specified key testing criteria into subtasks and accordingly forms the testing agent team .

% We supply the testing organizer agent with key testing criteria, summarized for different software applications. 
% {\HC This agent autonomously forms a testing team to cater to the varied and extensive testing requirements of different software types.}\Note{sc: one agent as a team?}

Once the test cases and generated code are ready, they are executed in the compiler, which functions as the environmental tool, producing execution logs. These logs clearly point out the gap between the generated code and the test cases. It shows satisfied testing requirements, existing function errors, and unmet testing requirements. This feedback information can be used to verify whether each agent's subtask is accomplished and guide the MAC network update.

\noindent\textbf{Updating team for textual back-propagation.}
The updating team consists of two collaborative agents: the gradient agent and the updating agent, adjusting the MAC network based on the execution logs, including the agent prompts and workflows. This process consists of two steps. First, the gradient agent summarizes the textual gradient by identifying accomplished subtasks for satisfied requirements, appending new subtasks for unmet requirements, and analyzing errors to detail their originating agents and revising suggestions. Second, the updating agent modifies the coding agent team by removing agents that have completed their subtasks, adding new agents for the new subtasks, and revising agent prompts to address issues identified in the previous generation. The agent workflow is updated once the agent team is revised, based on the dependencies among the subtasks.

% To increase flexibility, the MAC network is initialized in a self-organizing way. 
% into a sequence of smaller, more specific function implementation subtasks. By methodically addressing each simpler function completion task, the complex software development task can bedue to potential agent hallucinations, agents may make mistakes in completing each subtask, and the subtasks may not comprehensively address all the requirements.

% \noindent\textbf{Coding team for feed-forward.} In the feed-forward process, the coding team synthesizes code according to the given coding task. To handle the extensive software requirements, the coding team is implemented as a MAC network. It divides the comprehensive requirements into a sequence of smaller, more specific function implementation subtasks. By methodically addressing each simpler function completion task, the complex software development task can be progressively tackled, showcasing promising performance. 
% To increase flexibility, the MAC network is initialized in a self-organizing way. A coding organizer agent automatically decomposes the task requirements into subtasks and assembles the coding agent team accordingly. The number of coding agents is dynamic, adjusting in response to the task requirements. Note that, due to potential agent hallucinations, agents may make mistakes in completing each subtask, and the subtasks may not comprehensively address all the requirements. The quality of the generated code is unknown during the forward pass, which necessitates the self-evolving paradigm to iteratively refine the generation.

% {\HC Notably, the language agents demonstrate superior function completion capabilities, achieving over 90\% accuracy on benchmark HumanEval.} 
% \Note{sc: what is the difference between your coding team and previous works?}

==> EvoMAC/content/05-theoreticalanalysis.tex <==
\section{Theoratical Analysis}
To do:
\begin{equation}
    \label{to-prove}
    \setlength\abovedisplayskip{1pt}
    \setlength\belowdisplayskip{1pt}
    \begin{aligned}
        \mathcal{P}\left(\boldsymbol{r}_{n-1} \big | \boldsymbol{q}_{n-1}\right)  < \mathcal{P}\left(\mathbf{T}^{\mathcal{M}}_n (q_{n-1}) \in \mathcal{R}^+ \big | q_{n-1} \right) < (1 + \epsilon)  \mathcal{P}\left(\boldsymbol{r}_{n-1} \big | \boldsymbol{q}_{n-1}\right)
    \end{aligned}
\end{equation}


\begin{equation}
    \label{lemma}
    \setlength\abovedisplayskip{1pt}
    \setlength\belowdisplayskip{1pt}
    \begin{aligned}
        &\mathcal{P}\left(\mathbf{T}^{\mathcal{M}}_n (q_{n-1}) \in \mathcal{R}^+ \big | q_{n-1} \right) = \\
        &\sum_{\boldsymbol{q}_n} \mathcal{P}\left(\boldsymbol{r}_n \in \mathcal{R}^+ \big | \boldsymbol{q}_n \right) \sum_{\boldsymbol{r}_{n-1}}\mathcal{P}(\boldsymbol{r}_{n-1} \big | \boldsymbol{q}_{n-1}) \sum_{\boldsymbol{f}_{n-1}} \mathcal{P}(\boldsymbol{f}_{n-1} \big | \boldsymbol{r}_{n-1}) \mathcal{P}(\boldsymbol{q}_{n} \big | \boldsymbol{q}_{n-1}, \boldsymbol{f}_{n-1})
    \end{aligned}
\end{equation}
















% \begin{equation}
%     \label{lemma-a4-11}
%     \setlength\abovedisplayskip{1pt}
%     \setlength\belowdisplayskip{1pt}
%     \begin{aligned}
%         &\mathcal{P}\left(\mathbf{T}^{\mathcal{M}}_{n}(\boldsymbol{q}_{0}) \in \mathcal{R}^+ \big| \boldsymbol{q}_{0}\right)=\sum_{\boldsymbol{r_{n-1}}}\mathcal{P}(\boldsymbol{r}_{n-1}\big|\boldsymbol{q}_{n-1})\sum_{\boldsymbol{f}_{n-1}}\mathcal{P}(\boldsymbol{f}_{n-1} \big| \boldsymbol{r}_{n-1})\sum_{\boldsymbol{q}_{n}}\mathcal{P}\left( \boldsymbol{r}_{n} \in \mathcal{R}^+ \big| \boldsymbol{q}_{n}\right)\mathcal{P}(\boldsymbol{q}_{n} \big| \boldsymbol{q}_{n-1}, \boldsymbol{f}_{n-1})\\
%         &\geq\mathcal{P}\left(\mathbf{T}^{\mathcal{M}}_{n-1}(\boldsymbol{q}_{0}) \in \mathcal{R}^+ \big| \boldsymbol{q}_{0}\right)=\mathcal{P}(\boldsymbol{r}_{n-1}\in \mathcal{R}^+\big|\boldsymbol{q}_{n-1})
%         % &\geq\sum_{\boldsymbol{r}}\mathcal{P}(\boldsymbol{r}\big|\boldsymbol{q})\sum_{\boldsymbol{i}_k, k \in [N]}\prod_{j=1}^N\mathcal{P}(\boldsymbol{i}_j \big| \boldsymbol{i}_{j-1}, \ldots,\boldsymbol{i}_1,\boldsymbol{r})\cdot \sum_{\boldsymbol{c}_{k}, k \in [N]}\mathcal{P}(\boldsymbol{o}_{m}\in \mathcal{O}^+ \big| \boldsymbol{c}_{m}, \boldsymbol{q}, \boldsymbol{r})\prod_{k=1}^N\mathcal{P}(\boldsymbol{c}_{k} \big| \boldsymbol{i}_k, \boldsymbol{q})\\
%         % &=\sum_{\boldsymbol{r}}\mathcal{P}(\boldsymbol{r}\big|\boldsymbol{q})\sum_{\boldsymbol{i}_k, k \in [N]}\prod_{j=1}^N\mathcal{P}(\boldsymbol{i}_j \big| \boldsymbol{i}_{j-1}, \ldots,\boldsymbol{i}_1,\boldsymbol{r})\cdot \sum_{\boldsymbol{c}_{m}}\mathcal{P}(\boldsymbol{o}_{m} \in \mathcal{O}^+ \big| \boldsymbol{c}_{m}, \boldsymbol{q}, \boldsymbol{r})\mathcal{P}(\boldsymbol{c}_{m} \big| \boldsymbol{i}_m, \boldsymbol{q})
%     \end{aligned}
% \end{equation}

==> EvoMAC/content/06-experiments.tex <==
\vspace{-3mm}
\section{Experiments}
\vspace{-3mm}

\subsection{Experimental setup}
\vspace{-2mm}

\noindent\textbf{Baselines.} To validate the effectiveness of our EvoMAC, we conducted comparisons against both single-agent and multi-agent baselines. The single-agent baselines involve three prominent large models: GPT-4o-Mini (gpt-4o-mini), Claude-3.5-Sonnet (claude-3-5-sonnet-20240620), and Gemini (gemini-1.5-flash). For multi-agent baselines, we included five state-of-the-art (SOTA) methods: MetaGPT~\cite{metagpt2023}, Autogen~\cite{autogen2023}, Mapcoder~\cite{mapcoder2024}, Agentverse~\cite{agentverse2023}, and ChatDev~\cite{chatdev2023}. To ensure a fair comparison, all multi-agent baselines, including our EvoMAC, are powered by the efficient and powerful GPT-4o-Mini model. Additionally, to demonstrate the adaptability and robustness of our EvoMAC, we developed two EvoMAC variants using GPT-4o-Mini and Claude-3.5-Sonnet.

% To ensure a rigorous comparison, we equipped our system with  both GPT-4o-mini and Claude-3.5-sonnet.$\checkmark$

\noindent\textbf{Datasets.} Our experiments cover both the proposed rSDE-Bench and the standard coding benchmark HumanEval~\cite{humaneval2021}. HumanEval comprises 164 Python function completion problems, where the task is to generate code from a single function description. 
% Most problems are self-contained and can be solved within 100 lines of code.


% \noindent\textbf{Metrics.} Our rSDE-Bench uses accuracy as the evaluation metric, which quantifies the proportion of correctly fulfilled requirements relative to the total number of requirements via automatic test case verification. \Note{sc: should this be covered at the benchmark section?} It is similar to the pass@1 metric in HumanEval, which evaluates the pass ratio of correctly achieved functions against the total functions via unit test verification. To provide a comprehensive assessment, we involve the human expert evaluation, and the consistency and quality evaluation metrics defined in SRDD~\cite{chatdev2023}. 



\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/rSDE_evaluation.png}
    \vspace{-8mm}
\caption{Performance of four methods in terms of four evaluation metrics, including human evaluation, our automatic evaluation (accuracy), consistency, and quality. WB/GB and WA/GA represent Web/Game Basic and Web/Game Advanced respectively. Our accuracy metric is highly aligned with human evaluation across four dataset settings.} 
\label{Table:humanevalpercentage}
\vspace{-2mm}
\end{figure}
% The automatic evaluation metric reaches almost the same results as human evaluation, while the evaluation result from consistency and quality is not aligned with human evaluation.

% \begin{table}[!t]
% \centering
% \small
% \begin{tabular}{clcccc}
% \hline
% \multirow{2}{*}{Model}       & \multirow{2}{*}{Evaluator} & \multicolumn{2}{c}{\textbf{Game}}      & \multicolumn{2}{c}{\textbf{Website}} \\
%                              &                            & Basic         & Advanced      & Basic       & Advanced      \\ \hline
% \multirow{4}{*}{GPT-4o-mini} 
% & Human                      & 44.93         & 30.10         & 66.33        & 49.80            \\
% & Automatic                  & 42.76         & 30.10         & 62.90        & 44.40            \\
% & Consistency                & 0.8521        & 0.8521        & 0.8333       & 0.8333           \\
% & Quality                    & 0.5699        & 0.5699        & 0.03894      & 0.03894          \\\hline
% \multirow{4}{*}{MetaGPT}     
% & Human                      & 14.50         & 0.00          & 14.84        & 0.13             \\
% & Automatic                  & 16.67         & 0.00          & 15.41      	& 0.00             \\
% & Consistency                & 0.8334        & 0.8334        & 0.8306       & 0.8306           \\
% & Quality                    & 0.5566        & 0.5566        & 0.2216       & 0.2216           \\\hline
% \multirow{4}{*}{ChatDev}     
% & Human                      & 52.89 & 32.26  &            66.67 &	46.69               \\
% & Automatic                  & 53.63 & 32.23  &  62.67 & 43.45  \\
% & Consistency                & 0.8374        & 0.8374        &       0.8296      &   0.8296           \\
% & Quality                    & 0.558         & 0.558         &        0.8114     &      0.8114         \\\hline
% \multirow{4}{*}{EvoMAC}        
% & Human                      & 75.00  & 45.16       & 92.47            & 74.09              \\
% & Automatic                  & 76.09	& 54.84  & 89.38	& 65.05 \\
% & Consistency            &  0.8431       &0.8431  & 0.8407 &         0.8407      \\
% & Quality                    &    0.7374   &  0.7374  &  0.6535     &    0.6535        \\\hline
% \end{tabular}
% \end{table}

% \begin{table}[!t]
% \begin{tabular}{clcccc}
% \hline
% \multirow{2}{*}{Model}       & \multirow{2}{*}{Evaluator} & \multicolumn{2}{c}{\textbf{Game}}      & \multicolumn{2}{c}{\textbf{Website}} \\
%                              &                            & Basic         & Advanced      & Basic       & Advanced      \\ \hline
% \multirow{4}{*}{GPT-4o-Mini} 
% & Human                      & 44.93±20.54 & 30.10±13.03  &        66.33±4.04 & 49.80±4.87          \\
% & Automatic                  & 42.76±15.50 & 30.10±11.87  & 62.90±2.52 & 44.40±4.21 \\
% & Consistency                & 0.8521        & 0.8521        &       0.8333      &    0.8333           \\
% & Quality                    & 0.5699        & 0.5699        &        0.03894     &     0.03894          \\\hline
% \multirow{4}{*}{MetaGPT}     
% & Human                      & 14.50±1.02  & 0.00±0.00   &           14.84±0.43  & 	0.13±0.19       \\
% & Automatic                  & 16.67±2.72  & 0.00±0.00    & 15.41±0.00	& 0.00±0.00 \\
% & Consistency                & 0.8334        & 0.8334        &       0.8306      &     0.8306          \\
% & Quality                    & 0.5566        & 0.5566        &       0.2216      &     0.2216          \\\hline
% \multirow{4}{*}{ChatDev}     
% & Human                      & 52.89±11.41 & 32.26±7.90  &            66.67±0.58 &	46.69±1.82                \\
% & Automatic                  & 53.63±5.70 & 32.23±14.68  &  62.67±0.28 & 43.45±0.77  \\
% & Consistency                & 0.8374        & 0.8374        &       0.8296      &   0.8296           \\
% & Quality                    & 0.558         & 0.558         &        0.8114     &      0.8114         \\\hline
% \multirow{4}{*}{EvoMAC}        
% & Human                      & 75.00±4.61  & 45.16±0.00       &             &               \\
% & Automatic                  & 76.09±0.00	& 54.84±0.00  & 89.38±1.01	& 65.05±1.56 \\
% & Consistency            &  0.8431       &0.8431  & 0.8400 &         0.8400      \\
% & Quality                    &    0.7374   &  0.7374  &  0.6538     &    0.6538        \\\hline
% \end{tabular}
% \caption{Human evaluation results.} 
% \label{Table:humanevalpercentage}
% \end{table}

%%%%%%%%%%%%%%ORIGINAL DATA%%%%%%%%%%%%%%
% \begin{table}[!t]
% \begin{tabular}{clcccc}
% \hline
% \multirow{2}{*}{Model}       & \multirow{2}{*}{Evaluator} & \multicolumn{2}{c}{\textbf{Game}}      & \multicolumn{2}{c}{\textbf{Website}} \\
%                              &                            & Basic         & Advanced      & Basic       & Advanced      \\ \hline
% \multirow{4}{*}{GPT-4o-Mini} 
% & Human                      & 20.67±9.45/46 & 9.33±4.04/31  &                 193.67±11.81/292 & 123.0±12.03/247          \\
% & Automatic                  & 19.67±7.13/46 & 9.33±3.68/31  & 183.67±7.36/292 & 109.67±10.4/247 \\
% & Consistency                & 0.8521        & 0.8521        &       0.8333      &    0.8333           \\
% & Quality                    & 0.5699        & 0.5699        &        0.03894     &     0.03894          \\\hline
% \multirow{4}{*}{MetaGPT}     
% & Human                      & 6.67±0.47/46  & 0.0±0.0/31    &           43.33±1.25/292  & 	0.33±0.47/247      \\
% & Automatic                  & 7.67±1.25/46  & 0.0±0.0/31    & 45.0±0.0/292	& 0.0±0.0/247 \\
% & Consistency                & 0.8334        & 0.8334        &       0.8306      &     0.8306          \\
% & Quality                    & 0.5566        & 0.5566        &       0.2216      &     0.2216          \\\hline
% \multirow{4}{*}{ChatDev}     
% & Human                      & 24.33±5.25/46 & 10.0±2.45/31  &            194.67±1.7/292 &	115.33±4.5/247                \\
% & Automatic                  & 24.67±2.62/46 & 10.0±1.41/31  &  183.0±0.82/292 & 107.33±1.89/247  \\
% & Consistency                & 0.8374        & 0.8374        &       0.8296      &   0.8296           \\
% & Quality                    & 0.558         & 0.558         &        0.8114     &      0.8114         \\\hline
% \multirow{4}{*}{EvoMAC}        
% & Human  @yuchen                    & 34.5±2.12/46  & 14±0/31       &             &               \\
% & Automatic                  & 35.0±0.0/46	& 17.0±0.0/31  & 261.0±2.94/292	& 160.67±3.86/247 \\
% & Consistency @xiangrui           &  0.8431       &0.8431  & 0.8400 &         0.8400      \\
% & Quality  @xiangrui                  &    0.7374   &  0.7374  &  0.6538     &    0.6538        \\\hline
% \end{tabular}
% \caption{Human evaluation results.} 
% \label{Table:humaneval}
% \end{table}

% \begin{table}[!th]
% \centering
% \begin{tabular}{ccrrrr}
% \hline
%                               &   \multirow{2}{*}{Model}                & \multicolumn{2}{c}{\textbf{Game}} & \multicolumn{2}{c}{\textbf{Website}} \\ 
%                               &              & \multicolumn{1}{c}{Basic}     & \multicolumn{1}{c}{Advanced}     & \multicolumn{1}{c}{Basic}       & \multicolumn{1}{c}{Advanced}      \\ \hline
% \multirow{3}{*}{Single-Agent}
%                               & Gemini-1.5-flash  & 21.74±6.39	& 6.45±6.97   & 29.79±1.00	& 11.61±2.34  \\
%                               & Claude-3.5-sonnet & 44.20±5.41	& 18.29±13.26  & 58.90±1.48 & 37.11±1.06  \\ 
%                                & GPT-4o-Mini       & 42.76±15.50 & 30.10±11.87  & 62.90±2.52 & 44.40±4.21 \\\hline
% \multirow{6}{*}{Multi-Agent}  
%                               & MetaGPT           & 16.67±2.71	& 0.00±0.00   & 15.41±0.00	& 0.00±0.00  \\
%                               & Autogen           & 17.39±1.78	& 0.00±0.00   & 25.68±4.14	& 5.40±3.34  \\
%                               & MapCoder          & 29.71±6.72 &	7.52±6.10  & 34.70±1.59 & 14.57±0.66  \\
%                               & Agentverse        & 37.67±8.20	& 16.13±4.55  & 15.41±0.00	& 0.00±0.00  \\
%                               & ChatDev           & 53.63±5.70	& 32.26±4.55 &  62.67±0.28 & 43.45±0.77  \\\cline{2-6} 
%                               & EvoMAC              & \textbf{71.02±3.70}	& \textbf{41.94±5.26}  & \textbf{90.75±0.00}	& \textbf{67.21±0.00}   \\ \hline
% \end{tabular}
% \caption{Comparison with SOTAs.}
% \label{Table:sota game web percentage}
% \end{table}

%%%%%%%%%%%%%%ORIGINAL DATA%%%%%%%%%%%%%%
% \begin{table}[!th]
% \centering
% \begin{tabular}{ccrrrr}
% \hline
%                               &   \multirow{2}{*}{Model}                & \multicolumn{2}{c}{\textbf{Game}} & \multicolumn{2}{c}{\textbf{Website}} \\ 
%                               &              & \multicolumn{1}{c}{Basic}     & \multicolumn{1}{c}{Advanced}     & \multicolumn{1}{c}{Basic}       & \multicolumn{1}{c}{Advanced}      \\ \hline
% \multirow{3}{*}{Single-Agent}
%                               & Gemini-1.5-flash  & 10.0±2.94/46	& 2.0±2.16/31   & 87.0±2.94/292	& 28.67±5.79/247  \\
%                               & Claude-3.5-sonnet & 20.33±2.49/46	& 5.67±4.11/31  & 172.0±4.32/292 & 91.67±2.62/247  \\ 
%                                & GPT-4o-Mini       & 19.67±7.13/46 & 9.33±3.68/31  & 183.67±7.36/292 & 109.67±10.4/247 \\\hline
% \multirow{6}{*}{Multi-Agent}  
%                               & MetaGPT           & 7.67±1.25/46	& 0.0±0.0/31   & 45.0±0.0/292	& 0.0±0.0/247  \\
%                               & Autogen           & 8.0±0.82/46	& 0.0±0.0/31   & 75.0±12.08/292	& 13.33±8.26/247  \\
%                               & MapCoder          & 13.67±3.09/46 &	2.33±1.89/31  & 101.33±4.64/292 & 36.00±1.63/247  \\
%                               & Agentverse        & 17.33±3.77/46	& 5.0±1.41/31  & 45.0±0.0/292	& 0.0±0.0/247  \\
%                               & ChatDev           & 24.67±2.62/46	& 10.0±1.41/31 &  183.0±0.82/292 & 107.33±1.89/247  \\\cline{2-6} 
%                               & EvoMAC              & \textbf{32.67±1.7/46}	& \textbf{13.0±1.63/31}  & \textbf{265.0±0.0/292}	& \textbf{166.0±0.0/247}   \\ \hline
% \end{tabular}
% \caption{Comparison with SOTAs.}
% \label{Table:sota game web}
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[!t]
\vspace{-2mm}
\setlength{\arrayrulewidth}{0.05pt} 
\caption{Comparison of EvoMAC with five multi-agent and three single-agent SOTA baselines, all powered by GPT-4o-Mini. \textbf{\color{red}{Red}} values represent the percentage improvement of EvoMAC, shade in pink, over the single-agent baselines, shade in grey.} 
% \textbf{Bold} values indicate the best performance achieved across all methods for each task and benchmark., with respect to the rSDE-Bench and HumanEval tasks
\vspace{-3mm}
\centering
\scalebox{0.85}{
\begin{tabular}{c|c|cccc|c}
\hline

 &
   &
  \multicolumn{4}{c|}{\textbf{rSDE-Bench}} &
  \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}HumanEval\\ (\%)\end{tabular}}} \\

 &
   &
  \multicolumn{2}{c}{\textbf{Website(\%)}} &
  \multicolumn{2}{c|}{\textbf{Game(\%)}} &
   \\ 

\multirow{-3}{*}{\textbf{Method}} &
  \multirow{-3}{*}{\textbf{Model}} &
  Basic &
  \multicolumn{1}{c}{Advanced} &
  Basic &
  Advanced &
  Pass@1 \\ \hline
 &
  Gemini-1.5-Flash &
  29.79±1.00&
  \multicolumn{1}{c|}{11.61±2.34} &
  21.74±6.39 &
  6.45±6.97 &
  73.17 \\
 &
  Claude-3.5-Sonnet &
  58.90±1.48 &
  \multicolumn{1}{c|}{37.11±1.06} &
  44.20±5.41 &
  18.29±13.26 &
  89.02 \\

\multirow{-3}{*}{Single-Agent} &
  \cellcolor[HTML]{e6e6e6} GPT-4o-Mini &
   \cellcolor[HTML]{e6e6e6}62.90±2.52&
  \multicolumn{1}{c|}{\cellcolor[HTML]{e6e6e6}44.40±4.21} &
  \cellcolor[HTML]{e6e6e6}42.76±15.50 &
  \cellcolor[HTML]{e6e6e6}30.10±11.87 &
  \cellcolor[HTML]{e6e6e6}88.41 \\ \hline
 &
  MetaGPT &
   15.41±0.00 &
  \multicolumn{1}{c|}{0.00±0.00} &
  16.67±2.71 &
  0.00±0.00 &
  88.41 \\
 &
  Autogen &
  25.68±4.14 &
  \multicolumn{1}{c|}{5.40±3.34} &
  17.39±1.78 &
  0.00±0.00 &
  85.36 \\
 &
  MapCoder &
  34.70±1.59 &
  \multicolumn{1}{c|}{14.57±0.66} &
  29.71±6.72 &
  7.52±6.10 &
  90.85 \\
 &
  Agentverse &
   15.41±0.00 &
  \multicolumn{1}{c|}{0.00±0.00} &
  37.67±8.20 &
  16.13±4.55 &
  90.85 \\
\multirow{-3}{*}{Multi-Agent} &
  ChatDev &
  62.67±0.28 &
  43.45±0.77 &
 \multicolumn{1}{|c}{ 53.63±5.70}  &
  \multicolumn{1}{c|}{32.26±4.55}  &
  70.73 \\ \cline{2-7}
 &\cellcolor[HTML]{FFF7F7}
 &
 \cellcolor[HTML]{FFF7F7} \textbf{89.38±1.01} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF7F7}\textbf{65.05±1.56}} &
  \cellcolor[HTML]{FFF7F7}\textbf{77.54±2.04} &
  \cellcolor[HTML]{FFF7F7}\textbf{51.60±4.54} &
  \cellcolor[HTML]{FFF7F7}\textbf{94.51} \\

 &
  \multirow{-2}{*}{\cellcolor[HTML]{FFF7F7}EvoMAC} &
  {\color[HTML]{FF0000}\cellcolor[HTML]{FFF7F7}\textbf{+26.48}} &
  \multicolumn{1}{c|}{\color[HTML]{FF0000}\cellcolor[HTML]{FFF7F7}\textbf{+20.65}} &
  { \color[HTML]{FF0000}\cellcolor[HTML]{FFF7F7}\textbf{+34.78}} &
  { \color[HTML]{FF0000}\cellcolor[HTML]{FFF7F7}\textbf{+21.50}} &
  { \color[HTML]{FF0000}\cellcolor[HTML]{FFF7F7}\textbf{+6.10}} \\ \hline
\end{tabular}}
\label{Table:sota game web percentage}
\label{Tabel:sota humaneval}
\vspace{-6mm}
\end{table}


\vspace{-4mm}
\subsection{Effectiveness of rSDE-Bench's evaluation and EvoMAC}
\vspace{-2mm}
% To ensure the effectiveness of the human evaluation,  is evaluated by the same code engineer with the same standard, ensuring the . \Note{Do we need to say we get the output by log?}

\noindent\textbf{rSDE-Bench's automatic evaluation metric (accuracy) is highly aligned with human evaluation.}
Our primary goal is to validate the effectiveness of the proposed automatic evaluation in rSDE-Bench by comparing it with two existing evaluation metrics: consistency and quality, both from SRDD~\cite{chatdev2023}.
% Consistency is measured by the cosine embedding similarity between the requirements and the final code, while quality is calculated as the product of completeness (whether all functions are implemented with no "pass" statements), executability, and consistency.
% 替换掉Consistency measures the cosine embedding similarity between the requirements and the final code. Quality is calculated as the product of completeness (whether all functions are implemented with no "pass" statements), executability (whether the code runs without errors), and consistency. 
For a fair comparison, our golden standard is human evaluation, conducted by two expert code engineers who manually verify the fulfillment of requirements by interacting with the developed software. 
% 注释掉了For game, they play each game and test whether each game rule is achieved. For website, they browse each page and check whether both page elements and transition logic satisfy the requirement document. 
This process is tedious, taking around four hours per expert to evaluate the entire benchmark. The effectiveness of an evaluation metric depends on how closely it aligns with human evaluation.

% {\HC Accuracy serves as the outcome of the automatic evaluation metric used in rSDE-Bench. Each software development task comes with black-box test code that simulates human keyboard or mouse inputs to verify whether each requirement is correctly implemented. Note that, the automatic testing inevitably relies on the software logging intermediate states. We append the most simplified log requirements in the task requirements and minimize the load to the original software development.}\Note{sc: this should be covered at the benchmark section}


Fig.~\ref{Table:humanevalpercentage} presents the performance of four methods in terms of four evaluation metrics, including human evaluation, our automatic evaluation, consistency, and quality. 
We see that: i) our automatic evaluation is highly aligned with human evaluation across two software types (Website and Game), four methods, (GPT-4o-Mini, MetaGPT, ChatDev, and our EvoMAC), and two requirement difficulties (Basic and Advanced). The correlation coefficient between human evaluation and our accuracy metric is 0.9922, demonstrating the effectiveness of the proposed automatic evaluation in rSDE-Bench; ii) Consistency and quality metrics differ significantly from human evaluation, with correlation coefficients of 0.2583 and 0.3041, respectively.
This discrepancy occurs because consistency in SRDD measures similarity, and quality in SRDD focuses on executability, which does not guarantee that all requirements are met. This highlights the need for rSDE-Bench, as the SRDD benchmark does not support requirement-oriented software development.
% This shows that these metrics fail to accurately verify software requirement fulfillment.\Note{sc: why do they fail?} The existing benchmark SRDD could not support requirement-oriented software development, highlighting the necessity of our proposed rSDE-Bench.

% In summary, rSDE-Bench is the first requirement-oriented software development benchmark, enabling automatic and direct verification of requirement fulfillment.


\noindent\textbf{EvoMAC outperforms previous SOTAs on both software-level and function-level coding benchmarks: rSDE-Bench and HumanEval.} 
Tab.~\ref{Table:sota game web percentage} compares EvoMAC with five multi-agent and three single-agent SOTA baselines, all powered by GPT-4o-Mini for a fair comparison. We see that EvoMAC significantly outperforms previous SOTAs across all datasets. EvoMAC outperforms single-agent methods by 26.48\% on the rSDE-Bench Website Basic and 34.78\% on the rSDE-Bench Game Basic, as well as surpassing existing multi-agent methods by over 20\%. This highlights the effectiveness of multi-agent collaboration and the power of EvoMAC.


% outstands both single agent and SOTA multi-agent systems on function-level task HumanEval. It raises the accuracy to 94.51\% and gains 6.10\% more accuracy when compared to single agent. iii) EvoMAC is a reliable and universal method that outperforms previous SOTA multi-agent systems. The evolution mechanism equipped EvoMAC with the ability to better meet all requirements and avoid making mistakes.

% We also conduct experiments on function-level and simpler benchmark HumanEval. Results are shown in Tab.~\ref{Table:sota game web percentage}. All multi-agent systems are driven by GPT-4o-Mini for fairness. From the table we can see that EvoMAC still outperforms other SOTA coding multiagent systems on simpler function-level benchmark. All these experiments shows that EvoMAC is a reliable and universal method which outperforms previous SOTAs on both software-level and function-level coding benchmarks.

% \begin{table}[!t]
% \centering
% \begin{tabular}{cccccc|c}
% \hline
%                               & \multirow{3}{*}{Model} & \multicolumn{4}{c}{\textbf{rSDE-Bench}} & \multicolumn{1}{|c}{\multirow{2}{*}{\textbf{HumanEval}}}\\
%                               &              & \multicolumn{2}{c}{\textbf{Game}} & \multicolumn{2}{c}{\textbf{Website}} & \multicolumn{1}{|c}{} \\ 
%                               &              & \multicolumn{1}{c}{Basic}     & \multicolumn{1}{c}{Advanced}     & \multicolumn{1}{c}{Basic}       & \multicolumn{1}{c}{Advanced} & \multicolumn{1}{|c}{Pass@1}     \\ \hline
% \multirow{3}{*}{Single-Agent}
%                               & Gemini-1.5-flash  & 21.74	& 6.45   & 29.79	& 11.61  & 73.17\\
%                               & Claude-3.5-sonnet & 44.20	& 18.29  & 58.90 & 37.11  & 89.02\\ 
%                                & GPT-4o-Mini       & 42.76 & 30.10  & 62.90 & 44.40 & 88.41\\\hline
% \multirow{6}{*}{Multi-Agent}  
%                               & MetaGPT           & 16.67	& 0.00   & 15.41	& 0.00 & 88.41\\
%                               & Autogen           & 17.39	& 0.00   & 25.68	& 5.40  & 85.36\\
%                               & MapCoder          & 29.71 & 7.52  & 34.70 & 14.57  & 90.85\\
%                               & Agentverse        & 37.67	& 16.13  & 15.41	& 0.00  & 90.85\\
%                               & ChatDev           & 53.63	& 32.26 &  62.67 & 43.45  & 70.73 \\
%                               \cline{2-7} 
%                               & EvoMAC              & \textbf{71.02}	& \textbf{41.94}  & \textbf{90.75}	& \textbf{67.21} &    \textbf{94.51}\\ \hline
% \end{tabular}
% \caption{Comparison with SOTAs.}
% \label{Table:sota game web percentage}
% \end{table}


\vspace{-4mm}
\subsection{Effectiveness of evolving}
\vspace{-2mm}

Fig.~\ref{fig:evolving} shows the accuracy of EvoMAC over multiple evolving iterations on the rSDE-Bench and HumanEval. Each figure presents two curves: one for EvoMAC powered by GPT-4o-Mini (red) and the other by Claude-3.5 (blue). We have the following findings:

% To thoroughly validate the efficacy of the self-evolving, we conducted iterative reasoning experiments on rSDE-Bench and HumanEval with EvoMAC driven by two LLMs: 
% As depicted in Fig.~\ref{fig:evolving}, our EvoMAC demonstrates the following characteristics:



\begin{minipage}{0.6\textwidth}
\centering
\centering
\captionof{table}{Ablation study about coding/testing team with single/multi-agent, with/without evolving, and with/without environment tool. Best performances are bolded.}
\vspace{-2mm}
\setlength\tabcolsep{3pt}
\scalebox{0.8}{
\begin{tabular}{lcc|cc|cccc}
\toprule
\multirow{2}{*}{} & \multirow{2}{*}{Coding}                                                & \multirow{2}{*}{Testing}                                               & \multirow{2}{*}{Evol.} & \multirow{2}{*}{Env.} & \multicolumn{2}{c}{\textbf{Website(\%)}} & \multicolumn{2}{c}{\textbf{Game(\%)}} \\
                     &                                                                        &                                                                        &                           &                              & Basic             & Advanced         & Basic           & Advanced        \\ \midrule
a)                    & Single  & - & -                         & -                            & 63.70             & 41.70            & 42.76           & 30.10           \\
b)                    & Multi  & - & -                         & -                            & 67.47             & 39.27            & 68.10           & 41.93           \\
c)                    & Single  & Single  & $\checkmark$              & $\checkmark$                 & 80.82             & 60.32            & 71.73           & 41.93           \\
d)                    & Multi   & Single  & $\checkmark$              & $\checkmark$                 & 83.90             & 60.72            & 76.08           & 41.93           \\
e)                    & Single  & Multi   & $\checkmark$              & $\checkmark$                 & 83.56             & 61.94            & 73.91           & 45.16           \\
f)                    & Multi   & Multi  & $\checkmark$              & -                            & 78.08             & 52.23            & 55.80           & 33.32           \\
g)                    & Multi   & Multi   & $\checkmark$              & $\checkmark$                 & \textbf{90.75}    & \textbf{67.20}   & \textbf{77.54}  & \textbf{51.60}  \\ \bottomrule
\end{tabular}
\label{Table:ablation study}}
\vspace{-1mm}
\end{minipage}
\begin{minipage}{0.4\textwidth}
    % \begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/failure_cases.pdf}
    \vspace{-7mm}
    \captionof{figure}{Failure case distribution across evolving times on Website and Game.}
    \label{fig:failurecase}
% \end{figure}
\end{minipage}

\noindent\textbf{EvoMAC continuously improves with the evolving times.} Fig.~\ref{fig:evolving} shows that as evolving iterations increase, performance consistently improves across all five dataset settings, covering two difficulty levels, two software types, and both requirement-oriented and function complement benchmarks. This highlights the effectiveness, generalizability, and robustness of the self-evolving approach, encouraging EvoMAC to evolve whenever possible.


\noindent\textbf{EvoMAC indistinguishably improves with different driving LLM.} From Fig.~\ref{fig:evolving}, we see that: i) both EvoMAC variants continuously improve with evolving iterations, demonstrating the robustness of the self-evolving design; ii) the two curves do not intersect, indicating that the EvoMAC variant powered by a more powerful single model consistently outperforms the other, highlighting the advantage of using a stronger model. Success builds on success.

% Across both the software-level (rSDE-Bench) and the function-level (HumanEval) tasks, EvoMAC demonstrates a consistent optimization of its outputs with each successive reasoning iteration. This performance trajectory begins with a rapid ascent, akin to the steep learning curves observed in the early stages of neural network training, followed by a plateauing phase as the system approaches its optimal performance. This pattern closely mirrors the expected behavior of neural networks as they evolve through training epochs.

% \noindent\textbf{Universality Across Different LLM Drives.} Fig.~\ref{fig:evolving} (a-c) illustrate that regardless of the underlying LLMs, EvoMAC consistently exhibits the evolving characteristic of enhancing the quality of its outputs with each successive reasoning iteration. This observation highlights EvoMAC's universality across various LLMs for continuous performance improvement.

\noindent\textbf{Failure case analysis.} 
Fig.~\ref{fig:failurecase} shows the failure case statistics across iterations for Website and Game, showing a general decrease in errors as iterations progress. We see that: i) the most common errors are page display issues in Website and logic errors in Game; ii) page errors are resolved more quickly, while logic errors persist, suggesting that more isolated issues are easier to fix during the evolution process. This results in a sharp initial performance improvement as sipler problems are addressed early, followed by a plateau as more complex issues remain unresolved, shown in Fig.~\ref{fig:evolving}.


% In the website task, errors are reduced by nearly half by the 4th iteration, with page display being the most frequent and improved error type. In the game task, logical errors are the most common across all iterations. Syntax errors, though less frequent, are the most critical as they impair the overall executability of the code. Fortunately, these errors are fully resolved by the final iteration, highlighting the effectiveness of the evolving process in addressing major issues.


% \Note{actually the drop on game of EvoMAC the 50, biggest since the initial acc is too high} iv) Whatever the context length is, 

% \noindent\textbf{Multi-agent systems are not always superior to single-agent system.}
\vspace{-4mm}
\subsection{Ablation study}
\vspace{-2mm}

\begin{figure}[!t]
    \centering
    \begin{subfigure}{0.4\linewidth}
    \includegraphics[width=0.45\linewidth]{figures/evolving_times/iter_web_basic.png}
    \includegraphics[width=0.43\linewidth]{figures/evolving_times/iter_web_advanced.png}
    % \vspace{-2mm}
    \caption{Website}
    \label{fig:evolving-website}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.4\linewidth}
    \includegraphics[width=0.43\linewidth]{figures/evolving_times/iter_game_basic.png}
    \includegraphics[width=0.43\linewidth]{figures/evolving_times/iter_game_advanced.png}
    % \vspace{-2mm}
    \caption{Game}  
    \label{fig:evolving-game}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.18\linewidth}
    \includegraphics[width=1.0\linewidth]{figures/evolving_times/iter_humaneval.png}
    % \vspace{-2mm}
    \caption{HumanEval} 
    \label{fig:evolving-humaneval}
    \end{subfigure}
    \vspace{-3mm}
    \caption{Effect of EvoMAC performance across evolving times empowered by GPT-4o-Mini and Claude-3.5-Sonnet on Website, Game, and HumanEval datasets. The figure shows EvoMAC continuously improves with the evolving times on both LLM drives.}
    \label{fig:evolving}
    \vspace{-6mm}
\end{figure}



% To demonstrate the individual contributions of the coding team, testing team, and the evolving mechanism within the EvoMAC, we conducted a group of ablation studies in Tab.~\ref{Table:ablation study} to show the effectiveness of each component.

To assess the effectiveness of each component, Tab.~\ref{Table:ablation study} details an ablation study featuring seven EvoMAC variants. 
% This study explores the impacts of using single vs. multi-agent setups within the coding/testing teams and the inclusion or exclusion of an environment tool.

% {\HC \noindent\textbf{Effectiveness of evolving.} 
% Comparing Variant e) with Variant a) and Variant g) with Variant b), introducing self-evolving consistently leads to performance gains of 19.86\%/23.28\%, 20.24\%/27.93\%, 22.45\%/11.83\%, and 9.44\%/9.67\% for Website Basic and Advanced, and Game Basic and Advanced tasks, respectively. These improvements benefit both single-agent and multi-agent setups, demonstrating the effectiveness of evolving in enabling systems to adapt and refine their output through iterations, ultimately enhancing performance. } \Note{sc: repeat, REMOVE}


% 17.11\%/16.43\% and 18.62\%/21.45\% 
% EvoMAC enables multi-agent systems to evolve iteratively, leading to significant performance gains. For instance, compared to \textit{Ablation a}, \textit{Ablation c} shows a marked improvement in both website and game tasks, with basic website scores increasing by 17.12\% and basic game scores by 28.97\%. This demonstrates that evolving allows systems to adapt and refine their output through iterating, ultimately resulting in more robust and accurate performance. Thus, evolving is essential for achieving higher efficiency and task success in multi-agent systems.

\noindent\textbf{Effectiveness of objective environment feedback.}
Environment feedback, such as code execution logs, is essential for software development. Variant f) omits this tool, instead using an LLM-driven agent to critique the code. Comparing Variant g) with Variant f) shows a notable performance drop: Website tasks decrease by 12.67\% and 14.97\%, and Game tasks by 21.74\% and 18.28\% for Basic and Advanced levels, respectively. This underscores the importance of objective environmental feedback, as agent-driven critiques may introduce bias and fail to guide the evolution effectively.


\noindent\textbf{Effectiveness of multi-agent collaboration in coding team and testing team.} Comparing Variant g) to Variant e), we observe a performance decrease of 7.19\% and 5.26\% on Website Basic and Advanced respectively, when the coding team is reduced to a single agent. Similarly, comparing Variant g) to Variant d), there is a performance drop of 6.85\% and 6.48\% on Website Basic and Advanced respectively, also when the team is reduced to a single agent. These results demonstrate the necessary for involving multi-agent collaboration, highlighting that multi-agent setups offer more flexible adjustments and enhanced capabilities for evolution.

% The coding team establishes the initial foundation for subsequent iterations, while the testing team refines the model through rigorous evaluation and feedback. For instance, in comparison with \textit{Ablation g}, \textit{Ablation d} and \textit{Ablation e} show that the absence of the coding and testing team significantly influences the performance on both basic and advanced tasks.



% ** This stark contrast underscores the coding team's critical role in establishing a robust initial model. This enhancement suggests that the testing team's feedback loop is instrumental in fine-tuning the model and optimizing its performance.** 

% \noindent\textbf{Synergistic Effect of Coding Team and Testing Team.}
% The combined effect of the coding team and testing team is particularly noteworthy. When both modules are active, the EvoMAC outperforms all other configurations, indicating a synergistic effect. This finding highlights the importance of both the initial coding and subsequent testing phases in achieving optimal performance.




\begin{figure}[!t]
    \centering
    % \begin{subfigure}{0.49\linewidth}
    % \includegraphics[width=0.48\linewidth]{figures/web_bar_basic_3.png}
    % \includegraphics[width=0.48\linewidth]{figures/web_bar_advanced_3.png}
    % \vspace{-2mm}
    % \caption{Website}    
    % \end{subfigure}
    % \begin{subfigure}{0.49\linewidth}
    % \includegraphics[width=0.48\linewidth]{figures/game_bar_basic_3.png}
    % \includegraphics[width=0.48\linewidth]{figures/game_bar_advanced_3.png}
    % \vspace{-2mm}
    % \caption{Game}
    % \end{subfigure}
    % \vspace{-3mm}
    \includegraphics[width=0.95\linewidth]{figures/performance_token_dist.png}
    \vspace{-4mm}
    \caption{EvoMAC outperforms previous multi-agent and single-agent systems across all the context lengths across the four dataset settings on rSDE-Bench.}
    \vspace{-2mm}
    \label{fig:acc_dist}
\end{figure}

% \noindent\textbf{Accuracy decreases in long-context tasks.} Fig.~\ref{fig:acc_dist} shows that as task token length increases, both single-agent and multi-agent systems struggle to maintain accuracy.  We see that: i) as task token length increases, both single-agent and multi-agent systems struggle with accuracy, because longer contexts increase the likelihood of mistakes or missing key requirements; ii) ChatDev performs similarly to the single-agent GPT-4o-Mini, with accuracy dropping by 22.82\% for Website tasks and 45.14\% for game tasks, showing no advantage in handling long contexts.

% that single agent and existing multi-agent systems' performance drop sharply as context length increases on both website and Game tasks. Agents are likely to making mistakes or forgetting some important requirements when given a long context, thus resulting the performance drop.

\noindent\textbf{Effectiveness in handling varied task token lengths.} Fig.~\ref{fig:acc_dist} shows a comparison of task token lengths and performance across GPT-4o-Mini, ChatDev, and EvoMAC. We see that: i) EvoMAC consistently outperforms ChatDev and GPT-4o-Mini across all context lengths, with its self-evolving mechanism enabling the identification and correction of missed contexts and errors during iterations; ii) EvoMAC experiences less performance degradation on the rSDE-Bench Website than on the Game, as Website tasks are more modular and can be broken into subtasks, whereas Game tasks require more coordinated management, making them more challenging.

\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/case_study.png}
    \vspace{-6mm}
    \caption{We show the generated code of single-agent, GPT-4o-Mini, and multi-agent systems, ChatDev, and our EvoMAC (iteration =0/1) given the Website task (RecipeHub). After evolving, EvoMAC can revise previous issues and fulfill the task requirement.}
    \vspace{-6mm}
    \label{fig:casestudy}
\end{figure}


\vspace{-4mm}
\subsection{Case study}
\vspace{-2mm}

Fig.~\ref{fig:casestudy} presents the generated code by a single agent, GPT-4o-Mini, multi-agent systems, ChatDev, and our EvoMAC before and after evolving (iteration=0/1). We see that: i) EvoMAC after evolving can correct issues from previous iterations and successfully fulfill the task requirements; ii) multi-agent systems tend to better comprehend the task requirements and produce more well-structured code. More generated software can refer to Sec.~\ref{app:software} in the Appendix.


% \begin{table}[!ht]
% \centering
% \begin{tabular}{ccc}
% \hline
%                               &                   & HumanEval \\
%                               & Method             & Pass@1   \\ \hline
% \multirow{3}{*}{Single-Agent} & GPT-4o-Mini @xinyu      &   88.41     \\
%                               & Gemini-1.5-flash @xinyu &  73.17\\
%                               & Claude-3.5-sonnet @xinyu & 89.02\\ \hline
% \multirow{6}{*}{Multi-Agent}  & MapCoder @yaxin          & 90.85\\
%                               & MetaGPT  @yuchen         &  88.41\\
%                               & Autogen  @yuchen         &  85.36\\
%                               & Agentverse @xiangrui       & 90.85 \\
%                               & ChatDev  @zijie         & 70.73  \\ \cline{2-3} 
%                               & EvoMAC @xinyu &  \textbf{94.51}      \\ \hline
% \end{tabular}
% \caption{Comparison with SOTAs on HumanEval benchmark.}
% \label{Tabel:sota humaneval}
% \end{table}


% \begin{table}[]
% \begin{tabular}{cccrrrr}
% \hline
% \multirow{2}{*}{Coding Team} & \multirow{2}{*}{Testing Team} & \multirow{2}{*}{Evolving} & \multicolumn{2}{c}{Game} & \multicolumn{2}{c}{Website} \\
% &  &  & \multicolumn{1}{c}{Basic}     & \multicolumn{1}{c}{Advanced}     & \multicolumn{1}{c}{Basic}       & \multicolumn{1}{c}{Advanced}      \\ \hline
% - & -  & - & 19.67±7.13/46 & 9.33±3.68/31  & 183.67±7.36/292 & 109.67±10.4/247 \\
% \checkmark &      -                         &    -                       &   23.0±2.16/46	&8.67±2.62/31 &194.0±0.0/292	  & 94.0±0.0/247\\
% \checkmark &     \checkmark     &   -&31.33±3.3/46	& 12.67±0.47/31   & - &	-\\
%  \checkmark  &    \checkmark    &   \checkmark     &  32.67±1.7/46	& 13.0±1.63/31            &239.0±0.0/292	& 148.0±0.0/247   \\ \hline
% \end{tabular}
% \caption{Ablation of modules.}
% \end{table}


% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=0.5\linewidth]{figures/web_failure_case.pdf}
%     % \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
%     \caption{Failure case distribution v.s. evolving times. @yuchen}
%     \label{fig:failurecase}
% \end{figure}

% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=0.5\linewidth]{figures/game_failure_case.pdf}
%     % \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
%     \caption{Failure case distribution v.s. evolving times. @yuchen}
%     \label{fig:failurecase}
% \end{figure}


% \begin{figure}[!t]
%     \centering
%     \begin{subfigure}{0.3\linewidth}
%     \includegraphics[width=0.9\linewidth]{figures/web_failure_case.pdf}
%     \caption{Website}
%     \label{fig:web_failure_case}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.3\linewidth}
%     \includegraphics[width=0.9\linewidth]{figures/game_failure_case.pdf}
%     \caption{Game}  
%     \label{fig:game_failure_case}
%     \end{subfigure}
%     \caption{Failure case distribution across iteration times on website and game tasks.} 
%     \label{fig:failurecase}
% \end{figure}



% \begin{table}[!ht]
% \begin{tabular}{cccrrrr}
% \hline
% \multirow{2}{*}{Coding Team} & \multirow{2}{*}{Testing Team} & \multirow{2}{*}{Evolving} & \multicolumn{2}{c}{\textbf{Website}} & \multicolumn{2}{c}{\textbf{Game}} \\
% &  &  & \multicolumn{1}{c}{Basic}     & \multicolumn{1}{c}{Advanced}     & \multicolumn{1}{c}{Basic}       & \multicolumn{1}{c}{Advanced}      \\ \hline
% $\checkmark$ &  $\checkmark$  & $\checkmark$ &  258.0±0.0/292	& 159.0±0.0/247  &  -	& -  \\
% $\checkmark$  & -  & $\checkmark$ &  245.0±0.0/292	& 150.0±0.0/247  &  -	& -  \\
% -  & $\checkmark$  & $\checkmark$ &  244.0±0.0/292	& 153.0±0.0/247  &  -	& -  \\ 
% - &  -  & $\checkmark$ &  236.0±0.0/292	& 149.0±0.0/247  &  -	& - \\
% $\checkmark$ &  -  & - &  197.0±0.0/292	& 97.0±0.0/247  &  -	& - \\
% - &  -  & - &  186.0±0.0/292	& 103.0±0.0/247  &  -	& - \\
% \hline
% \end{tabular}
% \caption{Ablation of modules.}
% \end{table}

% \begin{table}[!ht]
% \begin{tabular}{ccrrrr}
% \hline
% \multicolumn{2}{c}{Evolving} & \multicolumn{2}{c}{\textbf{Website}} & \multicolumn{2}{c}{\textbf{Game}} \\
% \multicolumn{1}{c}{Gradient}     & \multicolumn{1}{c}{Update} & \multicolumn{1}{c}{Basic}     & \multicolumn{1}{c}{Advanced}     & \multicolumn{1}{c}{Basic}       & \multicolumn{1}{c}{Advanced}      \\ \hline
% W summary & W history &  -	& -  &  -	& - \\
% Wo summary & W history &  -	& -  &  -	& - \\
% W summary & Wo history &  -	& -  &  -	& - \\\hline
% \end{tabular}
% \caption{Ablation of gradient and updating.}
% \end{table}





==> EvoMAC/content/07-conclusion.tex <==
\vspace{-4mm}
\section{Conclusion}
\vspace{-3mm}

We propose EvoMAC, a novel self-evolving paradigm for MAC networks. EvoMAC iteratively adapts agents and their connections during the testing phase of each task. It achieves this with a novel textual back-propagation algorithm. EvoMAC can push coding capabilities beyond function-level tasks and into more complex, software-level development. Furthermore, we propose rSDE-Bench, a novel requirement-oriented software development benchmark. rSDE-Bench features both complex and diverse software requirements, as well as the automatic evaluation of requirement correctness. Comprehensive experiments validate that the automatic requirement-aware evaluation in rSDE-Bench aligns closely with human evaluation. EvoMAC outperforms previous SOTAs in both software-level rSDE-Bench and function-level HumanEval benchmarks. 
% \Note{sc: future works}

\noindent\textbf{Future works.} In the future, we plan to introduce a reward model to enhance the self-evolving paradigm's ability to learn from feedback and extend the rSDE-Bench to more software types. 

% integrate a reward model to enhance the general self-evolving paradigm's ability to learn from environmental feedback. Additionally, we plan to expand the rSDE-Bench to include a broader range of software types.

% In the future, we plan to apply the general self-evolving paradigm to more applications 

==> content/03-benchmark_old.tex <==
\section{RSD-Bench: Requirement-Oriented Software Development Benchmark}

% This section presents~\texttt{RSD-Bench}, a benchmark that targets to evaluate models on the task of generating codes to complete the software development requirements. To achieve comprehensive and objective evaluation, RSD-Bench features two typical realistic software types: game and website, and quantitative requirement-aware evaluation metrics. 
% The task formulation, benchmark construction, and features are introduced in the following Sec.~\ref{Benchmark:formulation},~\ref{Benchmark:construction}, and~\ref{Benchmark:features}. 
Generating code that precisely matches the defined software requirements is the cornerstone of a software development project. Therefore, to evaluate the capability of models to generate code that satisfies well-defined software requirements, we meticulously craft a benchmark~\texttt{RSD-Bench}. It encompasses the software requirements for two quintessential types of real-world software: games and websites. Additionally, it provides a rigorous and quantitative requirement-aware evaluation metrics for measuring how effectively generated code meets its intended objectives, thus aligning with the intricate demands of software engineering.


\begin{minipage}{0.4\textwidth}
% \begin{table}[]
\centering
\scalebox{0.65}{
\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{Benchmark} & \multicolumn{2}{c}{Software} & \multicolumn{2}{c}{Test Case} \\
                           & Amount   & Length  & Basic        & Advanced        \\ \midrule
Website                    & 45       &         1011/1553           &        292      &         247        \\ 
Game                       & 8        &         507/788           &        46      &         31        \\
\bottomrule
\end{tabular}}
\captionof{table}{Benchmark statistics}
\label{Table:benchmark_stat}
% \end{table}
\end{minipage}
\begin{minipage}{0.6\textwidth}
% \begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/combined_test_cases_with_format.pdf}
    % \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
    \captionof{figure}{Test case statistics of Game and Website tasks.}
    \label{Fig:testcase_dist}
% \end{figure}
\end{minipage}



\subsection{Benchmark construction}
\label{Benchmark:construction}

RSD-Bench includes two typical, real-world software types: games and websites, see Table.~\ref{Table:benchmark_stat}. The website benchmark is semi-automatically generated and scalable for large-scale expansion. The game benchmark is manually constructed, as each game has unique running rules, and its GUI is difficult to quantify, requiring human input to define measurable requirements. Both benchmarks follow a common two-step process to create high-quality task instances. After generating the task instances, we manually remove any unclear or unstable ones to ensure the benchmark's stability and measurability.

\noindent\textbf{Step 1: Software requirement generation.} Each task instance begins by generating clear and measurable software requirements. For the game benchmark, we focus on common real-world games and document detailed task requirements, including GUI layout initialization, interaction methods, expected game states, and game state logging. In addition to the game rules, we include game state logging as a requirement for automatic evaluation of the task. For the website benchmark, we start with a brief requirement that outlines the website’s workflow and then use large models to enrich the details following a predefined pattern. This approach ensures efficiency and scalability for the website benchmark.

\noindent\textbf{Step 2: Requirement-based test cases generation.} 
Each task instance incorporates black-box test cases to quantitatively evaluate the fulfillment of the generated software requirements. For the game benchmark, we manually create test cases, similar to the HumanEval~\cite{humaneval2021} code completion benchmark, which checks state changes based on specific inputs. In the game context, we assess game state changes in response to specific GUI interactions. For the website benchmark, large models are used to generate test cases based on the software requirements, followed by manual corrections to clarify any ambiguous cases.

\subsection{Benchmark formulation}
\label{Benchmark:formulation}

% The task is defined as generating codes to complete the software development requirements. Each task instance includes pairwise natural language-specified software requirements and associated test cases to evaluate the requirement completeness of the generated code.
% The task goal is to generate code given the natural language specified software requirement. Its input is the software requirement, and the evaluation is .


\noindent\textbf{Requirement-based model input.} A model is provided with clear and comprehensive software requirements. As depicted in Fig.~\ref{}, they are specified with natural language, which defines the software's targeted features and detailed workflows, rules, and states, such as interaction types and expected effects. These requirements are categorized into two levels of difficulty: basic and advanced, tailored to the complexity of each specific requirement. 
% We define two types of requirements: basic and advanced. 
% , RSD-bench designs software requirements for two types of software development tasks: games and websites. 
The basic requirements reflect the most fundamental capabilities, including software setup, keyboard control, clicking, and logging. The advanced requirements reflect more complex capabilities, including logical rules, and compositional effects. The model takes the software requirements as input to generate code. 

\noindent\textbf{Requirement-based evaluation metrics.} 
To evaluate the requirement completeness of the generated code, we associate black-box test cases (cf. Sec~\ref{Benchmark:construction}) with each defined software requirement. If the generated code can pass the test case, we consider the corresponding requirements are successfully achieved. The metric is the ratio of the passed test cases.

\subsection{Features}
\label{Benchmark:features}

\noindent\textbf{Complex and diverse software requirements.} Software development requirements in RSD-bench are typically long (averaging 507/1011 words for game and website benchmarks, respectively). Unlike existing function-level code completion and bug-fixing benchmarks, which focus on specific functions or issues, RSD-bench involves more complex and varied requirements, making it closer to real-world software development projects.

\noindent\textbf{Requirement-aware automatic evaluation.} Each task is automatically evaluated based on the pass rate of the requirements via running test cases. Existing software development benchmarks often define vague or unmeasurable requirements, relying on human evaluation or the similarity between generated code and requirements. These methods lack scalability and provide imprecise software performance evaluation. RSD-bench offers automatic, direct measurement of how well a task's software development goals are met.

\noindent\textbf{New and realistic software development challenges.} Solving tasks in RSD-bench demands: i) generating large codebases, ii) analyzing the fulfillment of each requirement, and iii) integrating code within a long context. This challenge requires advanced skills and knowledge typical of experienced software engineers, which are not commonly tested in traditional code generation benchmarks. These capabilities includes requirement analysis, task decomposition, code generation, testing, bug localization, and bug fixing.



==> content/05-theoreticalanalysis.tex <==
\section{Theoratical Analysis}
To do:
\begin{equation}
    \label{to-prove}
    \setlength\abovedisplayskip{1pt}
    \setlength\belowdisplayskip{1pt}
    \begin{aligned}
        \mathcal{P}\left(\boldsymbol{r}_{n-1} \big | \boldsymbol{q}_{n-1}\right)  < \mathcal{P}\left(\mathbf{T}^{\mathcal{M}}_n (q_{n-1}) \in \mathcal{R}^+ \big | q_{n-1} \right) < (1 + \epsilon)  \mathcal{P}\left(\boldsymbol{r}_{n-1} \big | \boldsymbol{q}_{n-1}\right)
    \end{aligned}
\end{equation}


\begin{equation}
    \label{lemma}
    \setlength\abovedisplayskip{1pt}
    \setlength\belowdisplayskip{1pt}
    \begin{aligned}
        &\mathcal{P}\left(\mathbf{T}^{\mathcal{M}}_n (q_{n-1}) \in \mathcal{R}^+ \big | q_{n-1} \right) = \\
        &\sum_{\boldsymbol{q}_n} \mathcal{P}\left(\boldsymbol{r}_n \in \mathcal{R}^+ \big | \boldsymbol{q}_n \right) \sum_{\boldsymbol{r}_{n-1}}\mathcal{P}(\boldsymbol{r}_{n-1} \big | \boldsymbol{q}_{n-1}) \sum_{\boldsymbol{f}_{n-1}} \mathcal{P}(\boldsymbol{f}_{n-1} \big | \boldsymbol{r}_{n-1}) \mathcal{P}(\boldsymbol{q}_{n} \big | \boldsymbol{q}_{n-1}, \boldsymbol{f}_{n-1})
    \end{aligned}
\end{equation}
















% \begin{equation}
%     \label{lemma-a4-11}
%     \setlength\abovedisplayskip{1pt}
%     \setlength\belowdisplayskip{1pt}
%     \begin{aligned}
%         &\mathcal{P}\left(\mathbf{T}^{\mathcal{M}}_{n}(\boldsymbol{q}_{0}) \in \mathcal{R}^+ \big| \boldsymbol{q}_{0}\right)=\sum_{\boldsymbol{r_{n-1}}}\mathcal{P}(\boldsymbol{r}_{n-1}\big|\boldsymbol{q}_{n-1})\sum_{\boldsymbol{f}_{n-1}}\mathcal{P}(\boldsymbol{f}_{n-1} \big| \boldsymbol{r}_{n-1})\sum_{\boldsymbol{q}_{n}}\mathcal{P}\left( \boldsymbol{r}_{n} \in \mathcal{R}^+ \big| \boldsymbol{q}_{n}\right)\mathcal{P}(\boldsymbol{q}_{n} \big| \boldsymbol{q}_{n-1}, \boldsymbol{f}_{n-1})\\
%         &\geq\mathcal{P}\left(\mathbf{T}^{\mathcal{M}}_{n-1}(\boldsymbol{q}_{0}) \in \mathcal{R}^+ \big| \boldsymbol{q}_{0}\right)=\mathcal{P}(\boldsymbol{r}_{n-1}\in \mathcal{R}^+\big|\boldsymbol{q}_{n-1})
%         % &\geq\sum_{\boldsymbol{r}}\mathcal{P}(\boldsymbol{r}\big|\boldsymbol{q})\sum_{\boldsymbol{i}_k, k \in [N]}\prod_{j=1}^N\mathcal{P}(\boldsymbol{i}_j \big| \boldsymbol{i}_{j-1}, \ldots,\boldsymbol{i}_1,\boldsymbol{r})\cdot \sum_{\boldsymbol{c}_{k}, k \in [N]}\mathcal{P}(\boldsymbol{o}_{m}\in \mathcal{O}^+ \big| \boldsymbol{c}_{m}, \boldsymbol{q}, \boldsymbol{r})\prod_{k=1}^N\mathcal{P}(\boldsymbol{c}_{k} \big| \boldsymbol{i}_k, \boldsymbol{q})\\
%         % &=\sum_{\boldsymbol{r}}\mathcal{P}(\boldsymbol{r}\big|\boldsymbol{q})\sum_{\boldsymbol{i}_k, k \in [N]}\prod_{j=1}^N\mathcal{P}(\boldsymbol{i}_j \big| \boldsymbol{i}_{j-1}, \ldots,\boldsymbol{i}_1,\boldsymbol{r})\cdot \sum_{\boldsymbol{c}_{m}}\mathcal{P}(\boldsymbol{o}_{m} \in \mathcal{O}^+ \big| \boldsymbol{c}_{m}, \boldsymbol{q}, \boldsymbol{r})\mathcal{P}(\boldsymbol{c}_{m} \big| \boldsymbol{i}_m, \boldsymbol{q})
%     \end{aligned}
% \end{equation}
